Better Peer Grading through Bayesian Inference

Peer grading systems aggregate noisy reports from multiple students to approximate a true grade as closely as possible. Most current systems either take the mean or median of reported grades; others aim to estimate students' grading accuracy under a probabilistic model. This paper extends the state of the art in the latter approach in three key ways: (1) recognizing that students can behave strategically (e.g., reporting grades close to the class average without doing the work); (2) appropriately handling censored data that arises from discrete-valued grading rubrics; and (3) using mixed integer programming to improve the interpretability of the grades assigned to students. We show how to make Bayesian inference practical in this model and evaluate our approach on both synthetic and real-world data obtained by using our implemented system in four large classes. These extensive experiments show that grade aggregation using our model accurately estimates true grades, students' likelihood of submitting uninformative grades, and the variation in their inherent grading error; we also characterize our models' robustness.

==> Better Peer Grading through Bayesian Inference (3)/PG5.tex <==

PG1 ignores the identities of each submission's authors. 
In practice, though, students' grades and grading abilities tend to correlate through their underlying abilities, time commitment, and interest in the course.
Piech et al's PG3 captured this correlation, which models graders' reliabilities as depending on their own submissions' grades in a deterministic way.
\citet{mi2015probabilistic} took this idea further with PG5, assuming that each grader's reliability is non-deterministically influenced by the true grade of their own submission---that is, that students with higher grades are often, but not always, better graders. 

\subsection{Revisiting PG5's Correlation Structure}
The PG5 model is defined only for classes with a single component. 
Abusing notation, let $s_u$ be the true grade of submission $u$ on its only component, and let $v(u)$ be the grader that authored submission $u$.
Then, the PG5 data generating process is:
\begin{alignat*}{2}
    \text{(True grades)}& \quad 
    s_u &&\sim \NormalDist(\mu_s, 1 / \tau_s); \\
    \text{(Reliabilities)}& \quad 
    \tau^{v(u)} &&\sim \NormalDist(s_u, 1 / \beta_0); \\
    \text{(Biases)}& \quad 
    b^v &&\sim \NormalDist(0, 1 / \tau_b); \\
    \text{(Peer grades)}& \quad
    g_u^v &&\sim \NormalDist(s_u + b^v, \lambda / \tau_v).
\end{alignat*}
Introducing this correlation structure has a computational drawback: while the true grade and bias Gibbs updates still have closed forms, the reliability update does not.
To get around this problem, Mi and Yeung use a discrete approximation of the reliability Gibbs update: they compute an unnormalized posterior probability for many potential values of a student's reliability, normalize these probabilities to sum to 1, and sample from the resulting distribution.
% (We use a similar approximation for our models that include correlation or censoring.)
Despite this computational difficulty, they show that this model better recovers staff grades on real peer grading data.

While it is possible to extend this %causal 
correlation structure to classes with multiple assignments or rubric elements---for example, by conditioning a student's reliability on the average of all of their submissions' true grades---the resulting model has a key flaw.
Because this model has an arrow from each true grade to the grader's reliability (a V-structure), observing a high true grade on one submission or rubric element increases the probability of \emph{lower} grades on the others.

We argue that these arrows should be flipped, as in Figure~\ref{fig:pg5}:
true grades should be modeled as conditionally dependent on their author's reliability rather than the reverse. 
This model still recovers PG5 in the single-submission, single-component case.  
Formally, our complete model is
\begin{alignat*}{2}
    \text{(Reliabilities)}& \quad 
    \tau^v &&\sim \NormalDist(\mu_s, 1 / \tau_s + 1 / \beta_0); \\
    \text{(True grades)}& \quad 
    s_{u,c} &&\sim \NormalDist\left(\frac{\tau_s \mu_s + \beta_0 \tau^{u(v)}}{\tau_s + \beta_0}, \frac{1}{\tau_s + \beta_0}\right); \\
    \text{(Biases)}& \quad 
    b^v &&\sim \NormalDist(0, 1/\tau_b); \\
    \text{(Effort probabilities)}& \quad 
    e^v &&\sim \BetaDist(\alpha_e, \beta_e); \\
    \text{(Efforts)}& \quad
    z_u^v &&\sim \Ber(e^v); \\
    \text{(Peer grades)}& \quad 
    g_{u,c}^v &&\sim \begin{cases}
        \NormalDist\left(s_{u,c} + b^v, \lambda / \tau^v\right) & z_u^v = 1; \\
        D_\ell, & z_u^v = 0.
    \end{cases}
\end{alignat*}
We also consider a censored version of this model, which adds reported grade variables that round each peer grade.

\begin{figure}
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=0.45\textwidth]{figures/graphical_model_pg5_original.pdf} &
        \includegraphics[width=0.45\textwidth]{figures/graphical_model_pg5_ours.pdf} \\
        (a) &
        (b)
    \end{tabular}
    \caption{(a) PG5's model of correlation between true grades and reliabilities. Conditioned on a student's reliability, their true grades are negatively correlated. (b) Our updated model. Conditioned on a student's reliability, their true grades are independent.}
    \label{fig:pg5}
\end{figure}

We include this feature in our experiments on real peer grading data in Appendix~\ref{sec: hyperparam_search} and \ref{sec: ablations_appendix}, where we show that correlation sometimes significantly hurts held-out likelihoods and is never a necessary feature of the best model. 

\subsection{Gibbs Updates (Without Censoring)}
Next, we provide Gibbs updates for the uncensored version of this model. 
First, notice that adding correlation between true grades and reliabilities has no effect on the bias, effort probability, and effort updates: because these updates condition on values of the reliability variables, the process by which these values are generated is irrelevant to the update rules.
The true grade update also has a closed form:
\begin{alignat*}{2}
    \text{(True grades)} &\quad
    \hat s_{u,c} &&\sim \NormalDist \left(
        \frac{\tau_s \mu_s + \beta_0 \hat \tau^{u(v)} + \sum_{v \in \matching_u} \hat \tau^v (g_{u,c}^v - \hat b^v)}{\tau_s + \beta_0 + \sum_{v \in \matching_u} \hat \tau^v},
        \frac{1}{\tau_s + \beta_0 + \sum_{v \in \matching_u} \hat \tau^v}
    \right).
\end{alignat*}
The reliability update, on the other hand, does not have a simple closed form.
Instead, as in our Gibbs updates for censored models, we make a discrete approximation, using the unnormalized posterior
\begin{align*}
    \text{(Reliabilities)} \quad
    \Pr(\tau^v | \bm{\hat s}, \bm{\hat b}, \bm{\hat z}, \bm{r})
    \propto 
    &\Pr(\tau^v | \mu_s, \tau_s, \beta_0)
    \cdot \prod_{u: v(u) = v} \Pr(\hat s_{u,c} | \tau^v, \mu_s, \tau_s, \beta_0) \\
    &\cdot \prod_{\substack{u \in \matching_v \\ z_u^v = 1}} \prod_{c=1}^C \varphi(g_{u,c}^v | \hat s_{u,c} + \hat b^v, 1 / \tau^v).
\end{align*}

\subsection{Gibbs Updates (With Censoring)}
Lastly, we add correlation to the fully featured model (with efforts and censoring).
As with the uncensored model, adding correlation has no impact on the bias, effort probability, or effort updates.
The remaining two, which still require discrete approximations, have the unnormalized posteriors
\begin{alignat*}{2}
    \text{(True grades)} &\quad
    \Pr(s_{u,c} | \bm{\hat \tau}, \bm{\hat b}, \bm{\hat z}, \bm{r}) 
    &&\propto \Pr(s_{u,c} | \hat \tau^{v(u)}, \mu_s, \tau_s, \beta_0) \prod_{v \in \matching_u} L(r_{u,c}^v | s_{u,c}, \hat \tau^v, \hat b^v, \hat z_u^v); \\
    \text{(Reliabilities)} &\quad
    \Pr(\tau^v | \bm{\hat s}, \bm{\hat b}, \bm{\hat z}, \bm{r})
    &&\propto \Pr(\tau^v | \mu_s, \tau_s, \beta_0)
    \cdot \prod_{u: v(u) = v} \Pr(\hat s_{u,c} | \tau^v, \mu_s, \tau_s, \beta_0) \\
    & &&\quad \cdot \prod_{u \in \matching_v} \prod_{c=1}^C L(r_{u,c}^v | \hat s_{u,c}, \hat \tau^v, b^v, \hat z_u^v)
\end{alignat*}


==> Better Peer Grading through Bayesian Inference (3)/abstract.tex <==
\begin{abstract}
Peer grading systems aggregate noisy reports from multiple students to approximate a ``true'' grade as closely as possible. Most current systems either take the mean or median of reported grades; others aim to estimate students’ grading accuracy under a probabilistic model. This paper extends the state of the art in the latter approach in three key ways: 
(1) recognizing that students can behave strategically (e.g., reporting grades close to the class average without doing the work); (2) appropriately handling censored data that arises from discrete-valued grading rubrics; and (3) using mixed integer programming to improve the interpretability of the grades assigned to students. We show how to make Bayesian inference practical in this model and evaluate our approach on both synthetic and real-world data obtained by using our implemented system in four large classes. These extensive experiments show that grade aggregation using our model accurately estimates true grades, students' likelihood of submitting uninformative grades, and the variation in their inherent grading error; we also characterize our models' robustness.

% old:
% Peer grading systems aggregate noisy reports from multiple students to approximate a "true" grade as closely as possible. Most current systems either take the mean or median of reported grades; others aim to estimate students’ grading accuracy under a probabilistic model. This paper extends the latter approach in four key ways: (1) allowing for more elaborate changes in student's grading accuracy over time; (2) recognizing that students can behave strategically (e.g., reporting grades close to the class average without doing the work); (3) leveraging the availability of scarce but trustworthy TA grades; and (4) appropriately handling censored data that arises from discrete-valued grading rubrics. We demonstrate how to make Bayesian inference practical in this model and evaluate our approach on both synthetic and real-world data. These extensive experiments show that grade aggregation using our model accurately estimates true grades, students' likelihood of submitting uninformative grades, and the variation in their inherent grading error; we also characterize our models' robustness.

\end{abstract}

==> Better Peer Grading through Bayesian Inference (3)/discussion.tex <==
% \gd{Preamble: we discuss the implications of our results for peer grading systems in practice.}
We have shown how probabilistic peer grading systems can be extended to provide incentives for effortful grading; to correctly model discrete peer grades; and to output discrete, interpretable final grades that approximate MAP estimates. We validated our models on four years of real classroom data and investigated both their ability to recover true parameters and their robustness on synthetic data. %We conclude with some remarks about putting our system into practice.

%\paragraph{Choosing hyperparameters.}
% \gd{not sure if this is a compelling discussion point -- it feels like a very obvious conclusion from the robustness experiments.}
Although the peer grading literature has repeatedly shown that Bayesian models can produce accurate grades, tuning them to produce such good performance can be a daunting task for an instructor---our model has 9 hyperparameters! Luckily, our robustness experiments in Section~\ref{sec:synthetic_robustness} showed that the model's posterior beliefs were robust to misspecifying the reliability, bias, and effort priors.
Two hyperparameters remain. The first is the true grade distribution, a choice that instructors often make when curving grades. The second is the specification of low-effort behavior, which is important both for boosting model performance and for disincentivizing bad behavior: if the model is good at identifying low effort behavior, students will exhibit this behavior less often. 
We recommend adapting the specification to capture low-effort behavior observed in spot checks. 

%Particularly in this latter case, our methodology of computing held-out likelihoods can help to validate that these hyperparameters have been set appropriately.

% \paragraph{Leveraging uncertainty estimates.}
Our insistence on providing uncertainty estimates is not just a statistical concern. 
Our methods work best when they are integrated into the design of the class, giving these uncertainty estimates pedagogical value.
For assignment grades, uncertainty estimates can direct TA spot checks towards areas of disagreement. 
For grader reliability, uncertainty estimates can inform whether students should be trusted to peer grade without TA supervision.
They can also help evaluate students' peer grading prowess: in our own class, we initialized the model to be confident that students had poor reliability and required students to do extra grading if the model's pessimistic estimate of their reliability was poor, but scored their peer grading based on the model's \textit{optimistic} reliability estimate. 
Thus, students got the best grade the model could justify, but students suspected to be weak got additional practice grading, which refined our reliability estimates in turn.

% In practice, courses using peer grading systems often have access to some trustworthy grades, either in the form of TAs (who are well calibrated and can be trusted to give relatively accurate grades) or gold-standard calibration submissions (which have been carefully graded by the course staff).
% \gd{Describe how they can be directed more productively by leveraging uncertainty estimates. TA spotchecks can be used on assignments with uncertain true grades, and students with uncertain reliability estimates can be asked to do more calibrations.}

% (old text on TA spotchecks
% TA spot checking can be helpful with incentives is to ask TAs to also evaluate the effort level of students who graded an spot checked submission. We expect that low-effort behavior should be fairly easy to detect by TAs. Therefore, in the threat of being spot checking by a TA is high enough, students would prefer not to report uninformative grades. for example, A common attack to peer grading systems is that students can reported high grades for their peers without carefully grading the assignments and avoid appeals in this way. This means that any peer grading system which cares about incentives should have a solution for this low-effort behavior. We proposed to use TA spot checking to make sure such behavior does not happen. If a low-effort student knows that by reporting a high grades, the chances of being spot checked increases, she would prefer not to do that. 

% Another dimension with which TA spot checking is helpful is with problematic cases. For example when the variance of reported grades are high, or when our model is really low confidant about the true quality of a submission. Diggin into such grading behavior that is outside out model can be really useful for our inference to make sure it updates its belief about the rest of the model parameters accordingly.

%\paragraph{Detecting low-effort grades.}
Our parameter recovery experiments in Section~\ref{sec:parameter_recovery} found that graders' effort probabilities were difficult to estimate: compared to reliabilities, effort probability estimates were much poorer with little data, and converged more slowly as data became available.
This is not a surprise: our low-effort graders choose grades that are as difficult as possible to distinguish from effortful graders.
The problem is exacerbated by coarse rubrics, which cause many high-effort grades to match the class average exactly.
Performance could be improved by tuning the specification of low effort behavior, using an autograding system as another unbiased signal about submissions' grades~\cite{han2020human}, or by leveraging other signals of low-effort behavior, such as graders' time spent grading and typing speed~\cite{wang2019improving}.
%Future work should evaluate such hybrid approaches.

% old text on incentives...
% \paragraph{The problem of reporting the mean.}
% We have already discussed that with the existance of apeals and TA spot checks, reporting too high or too low grades wtih a very risky move by a low effort grades. We also learn from the peer prediction literature cite[Hartline] that students look pretty reliable when they report the mean.
% % Jason Hartline: students look pretty reliable when they report the mean.
%  Our solution to avoid such a low effort behavior is to explicitly model this possibility and aviod it by assigning low dependability scores to it.

% All this shows is that under our grading scheme described above, and with the mechanism where TAs observe effort (partly based on signals that live outside the model like the text of a review) can do a pretty good job of incentizing efforts. 

% \paragraph{TA effort grades.} In addition to the standard use of TA grades to get better true grade estimates in a class (e.g., through estimating students' reliabilities better), BEM lets us use TAs in a class in a totally new dimension. In BEM, when assigned to grade an assignment, TAs are asked to report whether each student reported grade is high or low effort. TAs efforts grade can then be fed to the BEM inference and used to estimate true grades and student effort levels better in the course. We believe that doing such evaluation is an easy task for TAs relative to asking them to give a more course-grained grade to students grading performance. % Our experiments show that indeed such information can play an important role in estimating true grading in a way that is outside the power of other probabilistic models.




==> Better Peer Grading through Bayesian Inference (3)/existing_models.tex <==
We will use the following notation throughout the paper. 
Let $\submissions$ be the set of submissions and $\graders$ be the set of graders.
It is common for instructors to provide graders with a \emph{rubric}: a decomposition of the overall grade into a set of separate components. 
To capture this, we assume that each submission is graded on $C$ components $\components = \{1, 2, \dots, C\}$, with a maximum grade of $M$ for each.
Lastly, we write $\NormalDist(\mu, \sigma^2)$ to denote the normal distribution with mean $\mu$ and variance $\sigma^2$.

We now define PG1~\cite{piech2013tuned}, a key graphical model from the literature, which models students as having reliabilities and biases.
%(We modify their presentation slightly to allow grades to be split into multiple rubric components.)
The PG1 model supposes three sets of latent variables.
Each submission $u \in \submissions$ has a \emph{true grade} $s_{u,c} \in \mathds{R}$ for each rubric component $c \in \components$.
Each grader $v \in \graders$ is described by a \emph{reliability} $\tau^v \in \mathds{R}^+$, which captures the consistency of their grading, and a \emph{bias} $b^v \in \mathds{R}$, which describes their tendency to give generous or harsh grades.
An ideal grader would have a high reliability and 0 bias.
Then, when a grader $v$ grades a submission $u$, they give a peer grade $g_{u,c}^v \in \mathds{R}$ for each component $c$.
Concretely, the PG1 data generating process, depicted in Figure~\ref{fig:PG1_graphical_model}, is:
\begin{alignat*}{2}
    \text{(True grades)}& \quad 
    s_{u,c} &&\sim \mathcal{N}(\mu_s, 1 / \tau_s); \\
    \text{(Reliabilities)}& \quad 
    \tau^v &&\sim \GammaDist(\alpha_\tau, \beta_\tau); \\
    \text{(Biases)}& \quad 
    b^v &&\sim \mathcal{N}(0, 1 / \tau_b); \\
    \text{(Peer grades)}& \quad
    g_{u,c}^v &&\sim \mathcal{N}(s_{u,c} + b^v, 1 / \tau^v).
\end{alignat*}
This model has five hyperparameters: $\mu_s$ and $\tau_s$ fix the prior distribution of true grades; $\alpha_\tau$ and $\beta_\tau$ fix the prior over reliabilities (gamma-distributed to ensure that reliabilities are positive); and $\tau_b$ is the precision of the bias distribution.
% In this work, we also consider models without biases, which can easily be captured by clamping each grader's bias $b^v$ to zero.


\begin{figure}
    \centering
    \includegraphics[width=0.65\linewidth,trim={0 0.5cm 0 0}]{figures/graphical_model_pg1.pdf}
    \caption{The PG1 graphical model.}
    \label{fig:PG1_graphical_model}
\end{figure}

% Gibbs 
Armed with a dataset of peer grades, the goal of the model is to infer true grades for each submission and reliabilities and biases for each grader.
Such a complex model does not give rise to a closed-form expression for the posterior distribution over these parameters.
Instead, the posterior must be estimated numerically. 
A good option is \emph{Gibbs sampling}~\cite{Geman1984Gibbs}: initializing each variable randomly, repeatedly sampling new beliefs about a single variable in the model conditional on beliefs about all other variables, and reporting the long-run distributions of these samples. 
This approach is particularly attractive for PG1, as the true grade, bias, and reliability priors are conjugate priors for the normally-distributed peer grade likelihoods, giving each of the Gibbs updates a simple closed form.
We present these update equations in Appendix~\ref{sec: gibbs_updates}.

%\gd{Consider mentioning here that PG5 is interesting follow-up work that models correlations; we discuss it in-depth in the appendix.}



==> Better Peer Grading through Bayesian Inference (3)/figures/model_bem.tex <==
\tikz{
    \node[obs] (observed_grade) {$o_{u,c}^v$};
    \node[obs, dashed, below=0.6 of observed_grade] (reported_grade) {$r_{u,c}^v$};
    
    \node[latent,above=0.6 of observed_grade,xshift=-1.5cm] (true_grade) {$s_{u,c}$}; 
    \node[const, above=1.2 of true_grade, xshift=-0.3cm] (mu_s) {$\mu_s$}; 
    \node[const, above=1.2 of true_grade, xshift= 0.3cm] (sigma_s) {$\tau_s$};
    
    \node[latent,above=0.6 of observed_grade,xshift= 1.7cm] (effort) {$z_u^v$};
    \node[latent,above=0.8 of effort,xshift= 0cm] (effort_prob) {$e^v$};
    \node[const,above=0.8of effort_prob,xshift=-0.3cm] (alpha_e) {$\alpha_e$};
    \node[const,above=0.8of effort_prob,xshift= 0.3cm] (beta_e) {$\beta_e$};
    
    \node[latent,left=2 of effort_prob,xshift= 1cm] (reliability) {$\tau^v$};
    \node[const,above=0.8 of reliability,xshift=-0.3cm] (alpha_tau) {$\alpha_\tau$};
    \node[const,above=0.8 of reliability,xshift= 0.3cm] (beta_tau) {$\beta_\tau$};
    
    \node[const, left=2.5of observed_grade, yshift=1.0cm] (tau_l) {$\tau_\ell$};
    % plate
    % \plate [inner sep=.3cm,xshift=.02cm,yshift=.2cm] {assignment_plate} {(true_grade)} {\begin{tabular}{l}assignments $u$ \\ components $c$\end{tabular}};
    % \plate [inner sep=.3cm,xshift=.02cm,yshift=.2cm] {student_plate} {(reliability)(effort_prob)} {graders $v$};
    \plate [inner sep=.3cm] {c} {(true_grade)(observed_grade)(reported_grade)} {$c$};
    \plate [inner sep=.3cm] {u} {(true_grade)(observed_grade)(reported_grade)(effort)(c.north west)(c.south west)} {$u$};
    \plate [inner sep=.3cm] {v} {(reliability)(effort_prob)(effort)(observed_grade)(reported_grade)(u.south east)} {$v$};
    % edges
    \edge {mu_s, sigma_s} {true_grade}
    \edge {alpha_tau, beta_tau} {reliability}
    \edge {effort_prob} {effort}
    \edge {alpha_e, beta_e} {effort_prob}
    \edge {true_grade, reliability, effort, tau_l} {observed_grade}
    \edge {observed_grade} {reported_grade}
}



==> Better Peer Grading through Bayesian Inference (3)/figures/model_pg1.tex <==
\tikz{
    \node[obs] (observed_grade) {$o_{u,c}^v$};
    \node[obs, dashed, below=0.6 of observed_grade] (reported_grade) {$r_{u,c}^v$};
    
    \node[latent,above=0.6 of observed_grade,xshift=-1.2cm] (true_grade) {$s_{u,c}$}; 
    \node[const, above=0.8 of true_grade, xshift=-0.3cm] (mu_s) {$\mu_s$}; 
    \node[const, above=0.8 of true_grade, xshift= 0.3cm] (sigma_s) {$\sigma_s$};
    
    \node[latent,above=0.6 of observed_grade,xshift= 1.2cm] (reliability) {$\tau^v$};
    \node[const,above=0.8 of reliability,xshift=-0.3cm] (alpha_tau) {$\alpha_\tau$};
    \node[const,above=0.8 of reliability,xshift= 0.3cm] (beta_tau) {$\beta_\tau$};
    
    \node[latent,above=0.6 of observed_grade,xshift= 2.5cm] (bias) {$b^v$};
    \node[const,above=0.8 of bias,xshift=-0.3cm] (mu_b) {$\mu_b$};
    \node[const,above=0.8 of bias,xshift= 0.3cm] (sigma_b) {$\sigma_b$};
    % plate
    % \plate [inner sep=.3cm,xshift=.02cm,yshift=.2cm] {assignment_plate} {(true_grade)} {\begin{tabular}{l}assignments $u$ \\ components $c$\end{tabular}};
    % \plate [inner sep=.3cm,xshift=.02cm,yshift=.2cm] {student_plate} {(reliability)(bias)} {graders $v$};
    % alternative plates: include observed grade?
    \plate [inner sep=0.3cm] {assignment_plate} {(true_grade)(observed_grade)(reported_grade)} {$u$, $c$}
    \plate [inner sep=0.2cm] {student_plate} {(reliability)(bias)(observed_grade)(reported_grade)(assignment_plate.south east)(assignment_plate.north east)} {$v$}
    
    % \plate [inner sep=.3cm,xshift=.02cm,yshift=.2cm] {assignment_plate} {(observed_grade)(true_grade)} {\begin{tabular}{l}assignment $u$ \\ component $c$\end{tabular}};
    % \plate [inner sep=.3cm,xshift=.02cm,yshift=.2cm] {student_plate} {(observed_grade)(reliability)(bias)} {grader $v$};
    % edges
    \edge {mu_s, sigma_s} {true_grade}
    \edge {alpha_tau, beta_tau} {reliability}
    \edge {mu_b, sigma_b} {bias}
    \edge {true_grade, reliability, bias} {observed_grade}
    \edge {observed_grade} {reported_grade}
}



==> Better Peer Grading through Bayesian Inference (3)/intro.tex <==
%\gd{rough outline for now. Old text is commented out below in case it's useful.}

% peer grading is great
% - gives students exposure to others' work
% - lets instructors give frequent feedback and get frequent evaluations, even in large courses where TA grading is impractical.
Peer grading is a powerful pedagogical tool. 
It benefits students by giving them exposure to others' perspectives; helping them to internalize evaluation criteria by applying them critically to peer work~\cite{lu2012online}; and offering them feedback from equal-status learners~\cite{topping2009}.
Just as importantly, it gives instructors a way to make classes more scalable by shifting (some) grading workload away from course staff; effectively, this again benefits students, by giving them more opportunities for their work to be evaluated.

In order for peer grading systems to be both useful to instructors and acceptable to students, they must produce grades that are sufficiently similar to those that an instructor would have given. This is a challenging task because individual peer graders will be biased (consistently give generous or harsh grades); noisy (the same grader could grade an assignment differently on different days); and potentially strategic (some students will enter insincere peer grades unrelated to a submission's quality if they can get away with it). Addressing these interrelated challenges has been a topic of academic study in Computer Science for at least the last two decades. 

%\paragraph{Point-estimate methods}

The first methods for aggregating peer grades---and many others introduced more recently---produce \textit{point estimates} of each assignment's grade and each grader's quality
%Calibrated Peer Review (CPR) \cite{chapman01,robinson01} asks students to evaluate both instructor-provided ``calibration'' essays (for which correct grades are assumed to be known) and peer essays; the latter evaluations are weighted according to a student's calibration performance.
%
%Aropa \cite{hamer05} and CrowdGrader \cite{dealfaro14} assign grades as a weighted average of peer grades, assessing the quality of peer reviews as the peer grade's divergence from the average of peer grades rather than a calibration score. 
%\klb{Add a description along the same lines for} 
\citep{walsh2014peerrank,chakraborty2018incentivizing, prajapati2020swagrader,dealfaro14, hamer05}. 
%
%MechanicalTA \cite{wright2015mechanical} assigns grades as the median of peer grades, but leverages a pool of TAs to spot-check peer grades that appear to deserve a closer look.
%
%Various other systems assess review quality by asking students to provide explicit feedback on the reviews they received  \cite{gehringer01,cho05,mulder07,pare08}.
%\citet{kulkarni14} relies on similar feedback but also leverages algorithmic assessments of student submissions. %
%\gd{Original text said that they focused on ``incentivizing high effort grading''. What does this mean?}
%Finally, some systems use peer review as a mechanism for helping students to improve their work in response to feedback rather than grading a final product; examples include SWoRD \cite{cho05}, PRAZE \cite{mulder07}, and CaptainTeach \cite{politz14}. 
At their best, methods that produce point estimates %of grades and reliabilities
maximize the likelihood of the data given a model, e.g., by %work like expectation-maximization algorithms, 
assigning each grader a ``reliability'' parameter and iteratively updating these parameters to best describe the reported grades. (At worst, they do not even maximize likelihood. In this case they can produce grades and reliabilities that are inconsistent with each other, such as giving high weights to graders who are judged unreliable.)
%An advantage of such methods is that they produce final grades as simple functions of peer grades (e.g., a weighted average; a median), making the method easy to explain to students.
Even when they do maximize likelihood, such point estimates can be overly confident. This can matter for model accuracy: e.g., the data might show that only one of several students is reliable without offering evidence about which is which, making it likely that the model will commit to the wrong explanation. It can also limit the way such models are used in real classes: e.g., an instructor may not want to trust student grades until the system is \emph{confident} that a peer grader is reliable.

%\paragraph{Bayesian methods}
These problems can be addressed by inferring distributions over grade and reliability estimates rather than point estimates.  
% we see uncertainty estimates as a valuable output for instructors using peer grading systems, and so we do not evaluate these methods in this work. \gd{also mention that they handle discrete-valued grades inappropriately?}
A seminal paper due to \citet{piech2013tuned} introduced the first such system, using graphical models to simultaneously determine distributions over both grades for student submission and accuracy assessments for each grader.
%A variety of graphical models have been developed to aggregate peer grades in real class settings, accounting for increasingly complex grading behavior.
%We describe these models in technical detail in Section~\ref{sec:existing_models}, since they are the starting point for our own work, but survey them briefly here.
Their core ``PG1'' model assumes that  each assignment has a latent true grade and each peer grader has a latent bias and reliability; these parameters can be estimated from grading data through Bayesian inference, producing posterior distributions (and, hence, confidence intervals) on each assignment's grade and each student's grading abilities.
Piech et al.\ also introduced PG2 and PG3 models that respectively permit graders' biases to change over time and students' grading reliability to be correlated with their own assignments' grades.
Follow-up work by others further extended these models to allow for more complex reliability-grade correlations~\cite[the PG4 and PG5 models of][]{mi2015probabilistic} and to more explicitly account for differences between a single grader's reported grades~\cite[the PG6 and PG7 models of][]{wang2019improving}.
% KLB: try to avoid bringing the focus back to ourselves in related work section
% \gd{be more explicit about why we're basing our work on these models?}
% A core contribution of our work is to extend these existing graphical models to capture low-effort grading behaviour, handle discrete-valued rubrics, and explain the inferred  grades.

%\paragraph{Strategic behavior.}
A key issue in peer grading is that students are asked to expend effort in grading each other's work, and that it is difficult to assess whether they did expend this effort. For example, students can subvert systems that assess grading quality by comparing individual grades to each other if they coordinate on all reporting the same grade. In response to this issue, an extensive line of work in the mechanism design literature focuses on incentivizing high quality reporting in peer grading and other crowdsourcing environments~\cite{prelec2004bayesian,jurca2009mechanisms,jurca2005enforcing,faltings2012eliciting,witkowski2012robust,witkowski2013dwelling,radanovic2013robust,radanovic2014incentives,riley2014minimum,kamble2015truth,kong2016putting,shnayder2016informed, liu2018surrogate,goel2019deep, gao2019incentivizing,zarkoob2020report}. %\gd{Is it necessary to cite this much work? 7 lines of citations seems overkill. Maybe some of the earliest work and a survey paper would suffice...}.
Work in this area is mostly centered around the idea of \emph{peer prediction}, developing mechanisms that incentivize graders to grade the peer carefully by rewarding them based on comparing their peer grades to others'.  
While our model of low-effort grading is inspired by work in this area, these mechanisms typically rely on restrictive modeling assumptions, making them inappropriate for most practical peer grading systems. %\gd{is this true? if not, why can't we use these mechanisms in practice?}
% \gd{original text claimed that peer prediction work ``solely focuses on incentives and not grade aggregation; I don't really think that's true...}
Further, \citet{burrell2021measurement} found that rewards from out-of-the-box peer prediction mechanisms do not accurately reflect grader effort levels on realistic simulated data.


% We take a different, complementary approach to identifying low-effort behaviour, inferring graders' effort levels directly from their reported grades without leveraging any external information or automated grades. 
% We show that it is possible to detect some low-effort behavior only using reported grades. 
% Since we do not have access to such external information, we are unable to compare our results to theirs. \gd{this sounds defensive.} %\gd{phrase this more positively: we show that it is possible to detect some low-effort behaviour from the reported grades alone.}
% \hz{add Jason Hartline work here.}


% what's missing?
% - we argue that existing peer grading aggregation systems miss something.
% - first, graders are often strategic, avoiding costly grading if possible; should disincentivize such low-effort grading. 
% - second, grading rubrics are typically discrete, and forcing graders to pick discrete grades can create or mask disagreements.
% - third, AI systems produce black box grades to students, diminishing trust 
%   - \cite{kizilcec2016trust}: transparency in peer grading systems is key for trust
% - lastly, point-estimate methods don't give uncertainty estimates

% our contributions
% - we show that existing Bayesian models of peer grading can be augmented to handle all of these issues.
% - in particular, we show how the well-known PG1 model can incorporate an explicit model of low-effort behaviour and discrete-valued grades without making Gibbs intractable
% - we then show how to explain the posterior distribution as a weighted average using MIP
% - extensive experiments on real and synthetic datasets demonstrate that our additions to the model improve its fit to real peer grading behaviour, that the model is largely robust to incorrectly-set hyperparameters, and that the MIP explanations don't sacrifice much fidelity.




%When it is implemented in a course, or other structured learning environment, student work is evaluated by other  
% It helps students to learn better by , and can make classes more scalable by shifting 

% Many implementations of peer grading applications already exists~\cite{chapman01, de2014crowdgrader, wright2015mechanical}. When applied to assignments, each student work (submission) is given a final grade that depends only on peer evaluations. This presents the problem of grade aggregation -- how to distill the evaluations of several imperfect graders to a final grade that fairly reflects the quality of the submission. In this paper we assume that each student work has only one fair evaluation, which depends on the work's quality. Graders may have the following traits that prevent them from giving a submission the grade it deserves: (1) ... (2) ... (citations?)

Despite the considerable intellectual progress just described, there remain obstacles to deploying AI-based peer grading systems in practice. %We focus on three here. 
Statistically rich methods based on graphical models and economically informed mechanism design approaches have been developed independently; we are not aware of any system that unifies the two by providing both Bayesian parameter estimates and meaningful incentives for students to invest effort in peer grading. Furthermore, the statistical literature allows both students and the peer grading system itself to assign real-valued grades, whereas real instructors tend to use coarse-valued rubrics, particularly when eliciting grades from students. This can harm inference and also requires the instructor to find a way of mapping real-valued grades back onto their course's rubric. Even if this mapping produces accurate grades, students must be able to understand it in order to trust the system~\cite{kizilcec2016trust}.
%Third, complex grade aggregation methods are black boxes to students, often assigning grades that are accurate, but providing no reasoning for their decisions; assigning these opaque grades to students lowers their trust in the system~\cite{kizilcec2016trust}.

This paper addresses all of these problems, introducing extensions to probabilistic peer grading systems that can detect (and hence enable the disincentivization of) low-effort, strategic behavior by students; improve inference quality in the presence of discrete grading rubrics; and output interpretable, discrete final grades that closely approximate maximum a posteriori estimates. In what follows we begin by introducing notation and formally defining the baseline PG1 model (Section 2). We then introduce our novel methods for modeling grader effort, modeling discrete grade reports as censored observations, and outputting interpretable discrete grades via mixed-integer programming (Section 3). We evaluate our contributions in two ways. First, using real data from four offerings of a large class, we show that each of our effort and censoring model extensions improve likelihood on held-out data and that our method for generating interpretable grades closely tracks MAP estimates (Section 4). Second, using simulated data generated using the hyperparameters fit in the previous section, we assess our model's ability to recover grades and grader reliabilities as a function of dataset size and in the presence of hyperparameter misspecification (Section 5). We conclude by discussing ways in which our methods can be leveraged in the classroom (Section 6).\footnote{Open-source implementations of our models are available at \url{https://github.com/hezar1000/mta-inference-public}.}

% peer grading systems should:
% \begin{itemize}
%     \item account for low-effort grading behaviour
%             - peer prediction literature
%     \item allow for discrete-valued rubrics.
%             - studies (which?) have shown that peer graders need well-defined grading criteria, which often results in discrete-valued rubrics.
%             - we argue that handling these inappropriately can cause statistical issues, biasing estimates of grader quality and adding noise to grade estimates.
%     \item produce interpretable grades.
%             - transparency => trust in peer grading (cite)
%             - trust => more effective assessments (cite)
%     \item represent uncertainty about grades and graders.
%             - helps direct course staff's efforts.
% \end{itemize}



% this paper
% - address these problems by extending existing probabilistic models in the peer grading literature
% - we show that existing models can be extended to capture low-effort behaviour and discrete-valued rubrics, and that their outputs can be post-processed to produce transparent explanations
% - experiments on real data confirm that effort/discrete grades help, and explanations change few grades
% - follow-up on synthetic data to confirm accuracy and robustness 








% Peer grading is a powerful pedagogical tool.
% It helps students to learn better by thinking critically about the work of their peers and makes classes more scalable by shifting (part of) the grading workload from the course staff to students (citation).
% Any peer grading system that intends to works well in practice should assign students grades that reflect the true quality of their submitted work and also are easy to interpret. 
% %However, using peer grading in practice is often associated with two main concerns: aggregating reported grades and incentivizing high quality grading. 
% However, 
% %Many implementations of peer grading applications already exists~[cite Mechanical TA, Crowd grader, peer rank, etc]. 
% % Furthermore, the existence of low-effort grading behavior makes it difficult to properly aggregate peer grades into a final grade.
% % For example, straightforward methods of grade aggregation, such as taking the mean or median of the reported grades, could easily produce incorrect results when adding uncorrelated low-effort reports.
% %In these systems,
% reported grades by students in peer grading are not perfect. This is because (a) students' grading abilities can vary, e.g., they might be mis-calibrated graders, giving grades that are systematically higher or lower than an instructor's evaluation, (citation possibly) (2) students might be noisy graders due to the inherent difficulty of assessing the quality of piece of work submitted by their peers, and (3) students can behave strategically when grading each other (citation). 

% To estimate the true grade for assignments, most current practical peer grading systems either take the mean or median of reported grades (citations); some use iterative approaches\cite{walsh2014peerrank, de2014crowdgrader}, and other works aimed to estimate students’ grading accuracy under a probabilistic model (citations). Each of these approaches have their own pros and cons. Taking the mean or median is simple and straightforward, but often ignores the information hidden in students' heterogeneous ability in grading. Iterative approaches produce intepretable grades (final grade is the weighted average of reported grades), but they only provide point estimates of students' final grades and grading abilities without providing any intuition of how confident they are in each final grade. Probabilistic models provide much more information about students' grades and grading abilities but they usually have oversimplifying assumptions and final grades in these models are usually hard to interpret.  

% Furthermore, for a long time, the peer prediction and mechanism design literature have pointed out that in settings such as peer grading, if (strategic) students are not adequately incentivized to grade each other accurately, they would prefer to avoid paying the cost grading their peers accurately and report low effort and uninformative grades to the system. %a human experiment by \citet{gao2014trick} shows that such behavior can happen in practice. In a peer grading setting in 
% a notable way to adapt a low effort strategy in peer grading is to report the class average. \citet{hartline2020} argued that students can look moderately reliable when they report the class average. In our analysis on using peer grading in real class, we have in fact observed that some students who tend to always report grades that are close to class average more often that the class grade distribution suggests. This convinced us that such low-effort behavior exists and can harm the credibility of grades in the course. 

% In this work, we build upon the existing literature on probabilistic models for peer grading with an explicit emphasis on creating more practical grade aggregation methods. Most current graphical models attribute a latent bias and reliability parameter to each student, and a latent true grade to each assignment and estimates these parameters through Bayesian inference. The bias parameter specify the tendencies of individual students to be easy or hard graders; the reliability parameters model the inherent noise arising from each student's grading ability. However, they fail to identify strategic behavior, are designed for real-valued grades while the rubrics used in peer grading are often discrete valued, and often produce uninterpretable outputs. We extend these models to capture low-effort grading behavior, adapt their inference algorithms to handle discrete-valued rubrics, and design a post-processing step to produce more interpretable grades.





% %The most influential work in the area of probabilistic modeling for peer grading is that of \citet{piech2013tuned}, which proposes three closely related graphical models attributing a latent bias and reliability parameter to each student, and a latent true grade to each assignment and estimates these parameters through Bayesian inference. The bias parameters specify the tendencies of individual students to be easy or hard graders; the reliability parameters model the inherent noise arising from each student's grading ability.  Inspired by~\citet{piech2013tuned}, various follow-up work focused on designing modified models to improve predictive accuracy. Notable, cite[PG4 and PG5 authors] introduce two extensions that improve parameter estimation by making students reliability parameters depend of their grades on the same assignment. However, even after such improvements, there are certain problems associated with using the graphical modeling approaches in practice:  they fail to identify strategic behavior, are designed for real-valued grades while the rubrics used in peer grading are often discrete valued, and often produce uninterpretable outputs.

% \textbf{Discrete valued rubrics:} existing graphical models do not specifically count for the fact that grades are commonly discrete in peer gradin`g due to the usage of rubrics. One of the key components in practical peer grading systems is the use of grading rubrics. Usually, such rubrics are designed very carefully by the course instructors and are used by students to grade each other. An inherent result of using these rubrics is that (high effort) students need to map their observation of the true grades to one rubric element (i.e., bin their grades). Therefore, they only report a discrete grade to the system. To get better estimates of the true grades, a grade aggregation method should take such binning effect into account. Our experimental analysis shows that such a consideration indeed improves the accuracy of estimating the parameters of our model. 

% \textbf{Strategic behavior}
% Current graphical models do not consider strategic behavior. We therefore decided to particularly study cases where strategic students sometimes choose to grade each other carefully, but also sometimes choose to report the class average as their observed grade hoping that this behavior would remain undetected by the system. This choice is inspired by prior work in the peer prediction literature, which model students as making binary effort decisions and  aligns with our intuition that reporting grades which are lower than class average make it more likely for the given grade to get appealed, and reporting a grade that is higher than class average makes it more likely to get flagged as suspicious grading behavior by the course staff.

% %Inspired by prior work in the peer prediction literature, we model students as making binary effort decisions: we assume that when grading each other, students can either choose to be high effort, obtaining a noisy observation about the true grade of an assignment, or low effort, reporting the class average without grading the assignment. We depart from the theoretical peer prediction literature by building these effort decisions into a graphical probabilistic model. 
% We explain how such effort modeling can be integrated with existing probabilistic models and show that in the presence of low effort behavior, running inference considering efforts can recover true grades with more accuracy. %Our experimental analysis on simulated data shows that as the percentage of low effort behavior in a class increases, grade aggregation methods such as mean or PG1 indeed start to make large errors in estimating the true grades. However, BEM does a good job of detecting that behavior and filtering for that.
% Furthermore, when it comes to incentivizing high-quality grading, a key element is to have a reliable way to estimate students' grading performance in class. Our techniques give us an estimate of each graders effort, bias and reliability in the course. We multiply these three values to generate a so-called "dependability score" for each student in the course. Our experimental studies show that these dependability scores indeed have a high correlation with students grading performance in the class. Therefore, mapping them into (part of the total) grades in a course would provide a strong incentive to students to be accurate graders.

%  \textbf{Grade interpetability:} Unlike taking the mean, median or iterative approaches which provide as easy way for students to realize how their grades are computed (e.g., the weighted average of the reported grades), in probabilistic modeling approaches aggregated grades are hard to interpret because they are using samples taking from posterior distributions to come up with final grades. For the incentive mechanism to work at its best and a higher satisfaction level for students in a class, it is very important to make sure that students are able to interpret the grades given to them in class. Probabilistic grade aggregation methods, even though powerful, usually only act as a black box that outputs students' final grades. Such approaches usually rise a level of distrust and concern about where their grades are coming from and decrease their motivation. In this work, we introduce a novel mixed-integer programming formulation that acts as an extra layer on top of our approach that takes the samples resulting from running Gibbs sampling on our models as input and outputs estimated true grades that are a weighted average of students reported grades, where the weight are correlated with the effort and reliabilities of students who graded each assignment. 

% \textbf{Using uncertainity to direct spot checks:}

% %PG2 extends PG1 by assuming that the biases of students take a random walk as students do more grading. PG3 assumes that the reliabilities of students are correlated with their true grades.

% %Inspired by~\citet{piech2013tuned}, various follow-up work focused on designing modified models to improve predictive accuracy. --- talk about PG4-7.
% %In this work, we build upon the existing literature on probabilistic models for peer grading to create more practical grade aggregation methods. 

% % We address these challenges associated with using peer grading in practice through the lens of probabilistic modeling:

% %Finally, we also propose a new way to evaluate probabilistic models on real data. The main stream way to evaluate a grade aggregation method in the literature is to use a subset grades given by TAs/instructors as ground truth as see how good each model is at predicting these grades. We think that such approaches are not a practical way to compare models against each other since TAs and instructors can both be noisy grades as well. Instead, we propose to compare models based on how likely they make a subset of reported grades if that data was to be held-out in the inference phase. We think this is a better way to compare models with each other because it counts for the fact that TAs/instructors can be noisy too.  To our knowledge, we are the first to propose such real data evaluation strategy in the peer grading literature. 

% In what follows, we begin by describing a statistical approach to inferring assignment grades and grader reliabilities that roughly follows Piech et al and captures the current state of the art (Section 2). We show how to elaborate this model in three key ways: (1) to perform (better/more reliably?) when grades are discrete instead of continuous; (2) to account for the fact that students may follow low-effort strategies that existing models would otherwise interpret as reliable grading; (3) to allow for the existence of TA graders (who always make an effort) and calibration assignments (whose true grades are already known) to improve the system's estimates of both true grades on student assignments and student reliabilities (Section 3). In Section 4 we explain why this architecture offers good incentives, particularly when combined with an appeal mechanism and TA spot checking. In Section 5 we present experimental data that shows the quantitative performance of our system.































% However, if the existence of low effort behavior is not considered while aggregating the reported grades, the accuracy of aggregated true grades can potentially drop heavily.


 %A well-known and powerful statistical model introduced by~\citet{piech2013tuned} that is also the bases of our model in this work is called PG1. 

%For a peer grading system to be confidently used in practice, it needs to first motivates students to give high quality grades to each other. Then it need to aggregate the grades reported by students to come up with final grades, taking into account the inherent noise in students' grading ability and potential malicious behavior.

%In this work, 

% In this work, we design a grading framework with an emphasis on incentivizing high-effort grading. 
% Inspired by prior work in the peer prediction literature, we model students as making binary effort decisions: we assume that when grading each other, students can either choose to be high effort, obtaining a noisy observation about the true grade of an assignment, or low effort, reporting the class average without grading the assignment. 
% However, we depart from the theoretical peer prediction literature by building these effort decisions into a graphical probabilistic model. 
% The resulting model shares several similarities with existing work~\cite{piech2013tuned}, but instead of modeling each grader's intrinsic grading bias, it models their effort levels: the probability with which they play the high effort strategy while grading.
% We refer to this probabilistic model as the \textit{binary effort model (BEM)}. 
% We show how to use Gibbs sampling to run inference in this model to infer assignments' true grades and graders' noise and effort levels. 
% To our knowledge, our work is the first that uses a probabilistic model to capture an explicit notion of grading effort.
% % To the best of our knowledge, we are the first work that explicitly models effort in a probabilistic model are estimates that true running an inference which simultaneously tries to infer true grades, reliabilities and efforts in a class room.



% Using the BEM and running inference on it in a class has several advantages:

% (1) \textbf{Recovering True Grades:} 
% (2) \textbf{Grading the graders:} 


% In addition to explicitly modeling effort, BEM also introduces two other additional elements for peer grading:

% (3) 

% (4) 


    %  -- incentivize high quality grading
    %   -- grading the graders is important 
    %     -- cite Grant's work
    %     -- the grade should reflect both effort and accuracy cause the low effort stragegy exitst 
      
    %  -- grade aggregation accuracy
    %      -- mean and median are fine but igonore useful information. bayesian inference to the rescue
         
    % -- grade interpertability 
    %     -- students should be able to understad where their grades are commng from
        
    % -- handling discrete grades
    %  -- in peer grading grades are rubric based and this needs to be considered
     
    %  -- legerage TA grades to work better 
 
 %-- explain what our method does
 

 %Most current practical peer grading systems either take the mean or median of reported grades. Even though such simple approaches are shown to be powerful when recovering true grades, yet they do not have anything to say about the difference in grading performance by students in class. This information is important for two main reasons: (1) it can be help the grading aggregation percedure to put more weight on more dependable grades
% (2) it can also be used to incentivize students to provide high quality grading. 
 
%here is a line of work in the literature that focuses on inferring true grade and graders' reliabilities based students's grading behavior in class. However, such approaches have little to do with using the inferred information about student grading performance to incentivize high quality grading.  
 


%We start from a recent statistical approach and show how it can be advanced both to better model reality with a focus on designing incentives for students to put in the effort required for high quality grading, thereby bringing in many of the best ideas from the game theoretic literature.

%In order to incentivize high quality grading in a practical setting, it is important to be able to measure quality of the grading done by students. This not only helps with incentives, but also lets the grade aggregation to put more weight on higher quality grades.





%and to better reward good behavior and punish bad behavior, 



% \begin{comment}
% Introduction:
% Peer grading is a wonderful thing
% - helps students learn
%     - more frequent and faster feedback
%     - exposure to work at their own level of competence
%     - internalization of the rubric
% - helps manage large classes at lower cost

% The AI community has recognized the design of peer grading systems as an important problem of interest.

% There are two, somewhat interconnected strands of work in the literature:

% 1. statistical approaches (infer true grade, graders' reliabilities from students' joint reports)

% 2. peer prediction/mechanism design approaches (particular attention paid to the problem that students don't always have an incentive to report grades honestly; it's less work to do a superficial job grading)

% 3. of course, there are some lines of work that bring together both elements.

% We start from a recent statistical approach and show how it can be advanced both to better model reality and to better reward good behavior and punish bad behavior, thereby bringing in many of the best ideas from the game theoretic literature.

% In what follows, we begin by describing a statistical approach to inferring assignment grades and grader reliabilities that roughly follows Piech et al and captures the current state of the art (Section 2). We show how to elaborate this model in three key ways: (1) to perform more accurately when grades are discrete instead of continuous; (2) to account for the fact that students may follow low-effort strategies that existing models would otherwise interpret as reliable grading; (3) to allow for the existence of TA graders (who always make an effort) and calibration assignments (whose true grades are already known) to improve the system's estimates of both true grades on student assignments and student reliabilities (Section 3). In Section 4 we explain why this architecture offers good incentives, particularly when combined with an appeal mechanism and TA spot checking. In Section 5 we present experimental data that shows the quantitative performance of our system. .....
% \end{comment}







% A reliable peer grading system should:
% \begin{itemize}
%     \item \textbf{Educate} students on how to assign high quality grades 
%     \item \textbf{Incentivize} students to assign high quality grades
%     \item \textbf{Aggregate} reported grades by students in a way that makes the final grades of assignments close to their true values
%     \item \textbf{Evaluate} graders' performance, assigning reasonable grades students that reflect their actual performance
% \end{itemize}



% Current approaches in the literature to achieve these goals:

% \begin{itemize}
%     \item \textbf{Education}:  let students do calibration reviews
%     \item \textbf{Incentives}:  study spot checking suspicious behavior, including assignments with very high grades or very high variance between grades (Gao et al, Zarkoob et al)
%     \item \textbf{Aggregation}: aggregate grades by taking the median of reported grades. For spot checks, assigns TA grade instead, or, by using AI based approaches, (e.g., Piech, ...)
%     \item \textbf{Evaluation}: Assign full mark for grading performance if an student is not spot checked and TA grade for spot checked students. 
% \end{itemize}

% Flaws in the current approaches:
% \begin{itemize}
%     \item Grades are still noisy even after calibration
%     \begin{itemize}
%         \item Even though calibrations seems to be a powerful tool to increase students' grading reliability, data has shown that student graders can still be considerably noisy when grading. 
%         \item Taking the median could potentially devalue outliers, but data analysis has shown median grades can still end up giving grades that are not too low or too high. 
%         \item It would be much better if the aggregation could know which grades to trust more, e.g., could put more weight on more reliable grades.
%     \end{itemize}
%     \item Students can still get away by playing safe, i.e., reporting low effort but moderately high grades. 
%     \begin{itemize}
%         \item If grades are moderately high, risk of getting appealed is minimized
%         \item AI based approaches such as Piech et al do not consider low effort behavior in their analysis.
%         \item Spot checking is based on simple rules such as checking high variance grades or very high grades. So, moderately high grades are not likely to get spot checked.
%         \item There is need for a method that can detect (and punish) reporting low effort grades such as reporting moderately high grades.
%     \end{itemize}
%     \item Evaluating grader performance is very limited
%     \begin{itemize}
%         \item Current systems only learns about the grading quality of students that were spot checked, but it seems possible to learn about the quality of unchecked students (for example, by checking how closely they agree with the other graders).
%     \end{itemize}
% \end{itemize}

% In this work we focus on \textbf{Aggregation} and \textbf{Evaluate} in peer grading using Bayesian Inference when there is limited access to TA grades:
% \begin{itemize}
%     \item Modern peer grading systems such as Mechanical TA offer features such as calibration essays and TA spot checks
%     \item such features can be used to develop an integrated plan for reaching the properties mentioned above.
% \end{itemize} 

% We use these features along with Bayesian Inference to build a grade aggregation method that:
% \begin{itemize}
%     \item Aggregates grades accurately (define accurately?)
%     \begin{itemize}
%         \item finds estimates of true grades that could be interpreted as the weighted average of students' reported grades considering their effort and reliability.
%     \end{itemize} 
%     \item finds a dependability score for each student which tracks changes over students' effort and reliability over time.
%     \begin{itemize}
%         \item dependability score is a good proxy to for students' grading performance
%         \item they can be used to direct spot checking bad behavior or low quality grades more efficiently
%     \end{itemize}
% \end{itemize}

==> Better Peer Grading through Bayesian Inference (3)/methods.tex <==
We now present our main conceptual contributions.
First, we show how low-effort grading behavior can be disincentivized by augmenting the probabilistic model to include latent variables describing graders' \emph{effort}. 
Second, we show how to better handle the common case where graders select discrete grades from a coarse rubric by modeling these reports as \emph{censored} observations of an underlying real value. 
Third, we introduce a mixed-integer programming method for identifying \emph{interpretable} weighted averages of the peer grades that are faithful to the model's posterior beliefs.
We present and evaluate these features as extensions to PG1, which we found most applicable to our own class, but they could be applied to any of the PG* models in the literature. In Appendix~\ref{sec: PG5}, we show how these extensions could be added to the PG5 model of \citet{mi2015probabilistic}, additionally modeling correlations between students' submission grades and reliabilities.

%\gd{Maybe here point out that we present these as extensions to PG1, but they could be applied to any of the existing graphical models in the literature.}


\subsection{Modeling Grader Effort}
In order for a statistical model to be able to accurately recover true grades from peer reports, students must invest the effort required to grade as well as they can. Typically, students are incentivized to do so in part by receiving explicit grades for their peer grading prowess.  However, it is not easy to determine whether a student has done a good job of peer grading when there are no instructor or TA grades to which their evaluation can be compared. 
%
The main alternative method of providing an incentive---called peer prediction---is based on comparing students to each other. When all other students grade as accurately as they can, it is often possible to design reward systems that incentivize a given student to do the same (i.e., making effortful reporting an equilibrium). Unfortunately, however, other equilibria also exist in which students coordinate on the same grade without reading the assignment~\cite{jurca2009mechanisms, waggoner2014output, gao2014trick}. 
%, because the frequency distribution of grades is typically a bell curve centered around this point~\cite{hartline2020}.

% model
We can reduce students' incentives for such low-effort behavior by explicitly modeling it, helping us to avoid assigning high reliabilities to low-effort students. 
Each time a grader $v$ grades a submission $u$, we assume they make a binary decision about whether to make an \emph{effort} $z_u^v$ on the submission.
If they choose to make an effort, they produce a noisy grade as usual; otherwise, they choose a random grade from a fixed ``low-effort'' distribution $D_\ell$.
For simplicity, we model these effort decisions as being independent of the content of the submission.
Then, each student has an effort probability $e^v$, modeling their likelihood of exerting high effort when grading a submission.
Formally, adding this feature to PG1 produces the model: 
\begin{alignat*}{2}
    \text{(True grades)}& \quad 
    s_{u,c} &&\sim \mathcal{N}(\mu_s, 1 / \tau_s); \\
    \text{(Reliabilities)}& \quad 
    \tau^v &&\sim \GammaDist(\alpha_\tau, \beta_\tau); \\
    \text{(Biases)}& \quad 
    b^v &&\sim \mathcal{N}(0, 1 / \tau_b); \\
    \text{(Effort prob.)}& \quad 
    e^v &&\sim \BetaDist(\alpha_e, \beta_e); \\
    \text{(Efforts)}& \quad
    z_u^v &&\sim \Ber(e^v); \\
    \text{(Peer grades)}& \quad
    g_{u,c}^v &&\sim \begin{cases}
        \NormalDist(s_{u,c} + b^v, 1 / \tau^v), & z_u^v = 1; \\
        D_\ell, & z_u^v = 0.
        % \NormalDist(\mu_s, 1 / \tau_\ell),  & z_u^v = 0. \\
    \end{cases}
\end{alignat*}
Regardless of our choice of $D_\ell$, Gibbs sampling remains straightforward: both efforts and effort probabilities yield closed-form updates, and all other parameter updates simply exclude grades that a given sample calls low effort.

So, which low-effort distribution $D_\ell$ should we choose?
\citet{hartline2020} showed that the most robust ``low effort'' strategy is to report the class average, minimizing the expected distance to an effortful report. 
A point-mass low-effort model would be extremely brittle, so a natural $D_\ell$ is a normal distribution centered on the class average. 
We would also prefer to model idiosyncratic grading strategies as low effort, such as assigning everything a low or high grade, so that these outlying grades do not drive our reliability estimates.
Thus, our final $D_\ell$ is a mixture between this normal distribution and a uniform distribution: 
\begin{alignat*}{2}
    D_\ell = \begin{cases}
        \NormalDist(\mu_s, 1 / \tau_\ell), & \text{with probability } 1-\epsilon; \\
        \UniDist(0, M), & \text{with probability } \epsilon.
    \end{cases}
\end{alignat*}
%which is to say that low-effort students typically choose a random grade close to the class average, but still sometimes may choose to behave in a way that is not explained by the class average. 
Adding effort to a model introduces four new, tunable hyperparameters: $\alpha_e$ and $\beta_e$ parameterize a prior over graders' effort probabilities, which is beta-distributed to ensure that these probabilities are between $0$ and $1$; $\tau_\ell$ describes the amount of noise in graders' reports when they put in low effort; and $\epsilon$ specifies the probability with which a low-effort grader reports a grade uniformly at random. 

\subsection{Discrete Rubrics as Censored Observations}
% discrete-valued grades
In practice, submissions are usually graded on coarse, discrete rubrics such as five-point scales (and virtually no class allows graders arbitrary decimal precision).
PG1 and all of its successors nevertheless assume that reported grades are real valued. They do this for two good reasons. First, continuous distributions like Gaussians are realistic models of true grade distributions, and arguably reported grades are just discretizations of the same continuous values. 
Second, most discretizations produce non-conjugate priors, making Gibbs updates computationally intractable.

However, failing to model grades as discrete-valued can skew a model's posterior beliefs. 
Treating discrete grades as real-valued can add statistical bias to graders' reliability estimates, both by overestimating (e.g., graders appear to be in perfect agreement when their rounded grades are interpreted as draws from a continuous distribution) or underestimating (e.g., graders can appear to disagree substantially after rounding, even if they correctly assess that a true grade is close to the midpoint between two integers). Of course, degraded reliability estimates lead to degraded true grade estimates.

% censoring
We propose an approach for extending PG-style models to realistic discrete grade distributions that maintains the tractability of Gibbs updates.
Let $G \subset \mathds{Z}$ be a set of legal discrete grades (e.g., integers between $0$ and $5$), and let $n_G: \mathds{R} \to G$ be a function mapping a grade to its nearest value in $G$, rounding up.
We continue to model a grader $v$ grading a submission $u$ as sampling a real-valued peer grade $g^v_{u,c}$, %from a Gaussian centered on $u$'s true grade plus $v$'s bias term $b^v$ and with variance equal to $v$'s reliability $\tau^v$. 
but we now treat these real-valued peer grades as latent variables, with the student reporting the discrete grade $r_{u,c}^v = n_G(g^v_{u,c})$: 
a \emph{censored observation} of the real-valued peer grade.
% Note that although graders' reports are discrete, the underlying true grades are still continuous in this model.
Figure~\ref{fig:graphical_model} shows the resulting graphical model. %, including biases, efforts, and censoring.
Observe that it correctly leads us to consider grader disagreement to be more likely when an assignment's true grade is 3.51 than when it is 3.0.

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth,trim={0 0.5cm 0 0}]{figures/graphical_model_full.pdf}
    \caption{Our complete graphical model.}
    \label{fig:graphical_model}
\end{figure}

% closed-form Gibbs updates
Naive Gibbs sampling would be extremely inefficient for this model: the posterior distribution has multiple modes where the true grade nearly matches one latent peer grade, and Gibbs sampling rarely moves between these modes.
To avoid this problem, we instead marginalize over peer grades, integrating over all of their possible values.
Although the Gibbs updates no longer have closed-form expressions, there is an efficient discrete approximation.
First, notice that we can still straightforwardly compute the likelihood of a reported grade for any setting of the submission's true grade and the grader's reliability and bias.
Then, to update a true grade variable, we consider a uniform grid of possible grades (ranging from 0 to a grade slightly above the maximum grade $M$), compute an unnormalized posterior probability for each value, renormalize these probabilities to sum to 1, and sample from the resulting discrete distribution.
The reliability and bias updates are similar, testing uniform grids of plausible reliabilities and biases.
We provide full details of these Gibbs updates in Appendix~\ref{sec: gibbs_updates}.

\subsection{Explaining Discrete Grades via MIP}

A key advantage of a Bayesian approach to reasoning about peer grades is that it yields distributional posterior beliefs about each quantity of interest rather than point estimates. However, students still expect to receive discrete grades rather than probability distributions. Furthermore, if the course staff grade on the same rubric as the students, assigning real-valued grades to students incentivizes half of them to ask for regrades (e.g., if their true grade is 3.6, the rounded TA grade would be 4). How should we turn posterior distributions into discrete grades? 
One might map the mean of the Gibbs samples to the nearest rubric element, but this can lead to rounding errors. A better option is to choose the rubric element corresponding to the continuous grade interval having the highest mass in the posterior distribution---the \emph{maximum a posteriori (MAP)} grade. While this approach is statistically sensible, it leaves students with little insight about how their peer grades influenced the calculation; this can lead to reduced trust in the system~\cite{kizilcec2016trust} and more appeals. %\gd{and making their incentives unclear? though I'm not sure that interpretable grades help incentives because the weights still come from a black box.}

Both approaches have an additional problem: they sometimes produce final grades larger or smaller than any peer grade (e.g., when the model assigns biases having the same sign to all graders). In our experience, students find such grades confusing and unfair; they instead expect to receive final grades that interpolate their received grades, such as averages weighted by each grader's perceived trustworthiness.
Students also tend to fixate on low-quality peer reviews, strongly preferring such reviews to have no impact on their final grade rather than a small impact.

We propose a novel mixed integer programming (MIP) formulation that maps posterior grade distributions to discrete final grades that can be explained as rounded weighted averages of reported peer grades.
To start, we assign a weight for each grader in proportion to their reliability and effort estimates.
The MIP then adjusts these weights in two ways to maximize the posterior probability of the resulting rounded weighted average.
First, we allow the MIP to deviate from each grader's initial weight by up to a constant $S$ to improve the likelihood of the resulting rounded grade. 
Second, we require the MIP to assign weights either equal to zero or above a minimum threshold $T$, avoiding small, non-zero weights on relatively uninformative grades.
Notice that the resulting weighted averages can never produce a grade outside of the range of the peer grades.
%\gd{note for the future: consider penalizing the distance a grade is rounded to avoid producing weighted averages close to a bin boundary. need to be careful to set penalty coefficients appropriately (especially since there's a grade-rounding penalty and a weight-changing penalty); maybe look for smallest difference between two adjacent bins' likelihoods. would also be nice to have L2 loss so that changing everyone's weight a little is better than changing one grader's weight a lot.}
%we set these desired weights in proportion to our estimates of the peer graders' reliabilities $\tau^v$ and effort draws $z_u^v$ on submission $u$, giving higher weights to trustworthy graders.
%\klb{This breaks ties among equally likely weighted averages and also restricts the set of possible final grades to those that are reflected by more informative grade.}
%To break ties among equally likely weighted averages \gd{this doesn't only break ties -- it restricts the set of possible final grades!}, 
We define our MIP formulation formally in the Appendix~\ref{sec: mip}.


%After running any of these Gibbs sampling methods, a lingering issue is that we must aggregate these samples to decide upon a grade for each submission.
%Ordinarily, a common method is 
%the mean of the Gibbs samples. If necessary, we can round this to the nearest rubric element, but this still can incentivize undesired behavior: students might then appeal their grades, hoping that a TA re-grading their submission would round their grade up to the nearest discrete value on the rubric.
%Second, even after rounding the sample mean to a discrete grade, it is difficult for students to understand how their grades were calculated or which of their peer grades influenced the calculation, leading to distrust in the peer grading system. \gd{and making their incentives unclear? though I'm not sure that interpretable grades help incentives because the weights still come from a black box.}


%and furthermore students want understandable explanations of the relationship between their peer grades and their final grades.

% \klb{This section needs some serious work. There should be a paragraph listing desiderata (things we want to hold true of a student's final grade) followed by our solution and why it achieves each desideratum. Right now the motivation is quite decoupled from the solution. We introduce problems that we may not have solved (such as a desire to request regrades through a belief that rounding will help)---if indeed we solved this, it's not clear. There's confusion about whether our methods are important only in the case where output grades need to be discrete or whether they'd help in the real-valued case too. And there are a bunch of properties of the solution that aren't motivated in the setup at all (why the desired weights? why have $S$, and how should it be set? why threshold small weights?). I did some work on this but ultimately I think you guys need to take another pass first.}

% \gd{Too tired to rewrite now, but the plan is: 
% - Discrete rubrics have another subtle problem: students who get a final grade just below a discrete value will tend to gain marks from asking for a regrade. Can fix this by allowing course staff to assign partial marks, but we'd rather give a discrete grade: students are already thinking on this scale and it's helpful to see where their own work fits into the scale.
% - There are several methods for producing a discrete-valued grade (take the mean of the Gibbs samples and round it; or round each Gibbs sample and take the mode), but this leaves students feeling like their grade came from a black box.
% - Since we already have estimates of each grader's quality (reliability, effort, bias), insist on basing explanations on these
% - Want to give simple explanations: insist that we represent final grade as a weighted average, and that this weighted average never puts small, non-zero weights  
% }

%The most obvious place to begin is with 
%After running any of these Gibbs sampling methods, a lingering issue is that we must aggregate these samples to decide upon a grade for each submission.
%Ordinarily, a common method is 
%the mean of the Gibbs samples. If necessary, we can round this to the nearest rubric element, but this still can incentivize undesired behavior: students might then appeal their grades, hoping that a TA re-grading their submission would round their grade up to the nearest discrete value on the rubric.
%Second, even after rounding the sample mean to a discrete grade, it is difficult for students to understand how their grades were calculated or which of their peer grades influenced the calculation, leading to distrust in the peer grading system. \gd{and making their incentives unclear? though I'm not sure that interpretable grades help incentives because the weights still come from a black box.}


==> Better Peer Grading through Bayesian Inference (3)/old/evals.tex <==
\textbf{Question:} What kind of evaluations are needed to convince ourselves and others that the Bayesian inference method is a reliable tool to use in a real course. 

% Note: we might actually want to evaluate our inference WITHOUT TA's separately from TA's effect (or optimal spotchecking methods) - Lena

\subsection{Synthetic data experiments}

\textbf{Question:} How accurate are the estimates of true grades and dependabilities using synthetic data in a CPSC430 like environment (~100 students and 4 grades per assignment)? what are the driving factor\\

\textbf{Sample Answer:} 
\begin{itemize}
    \item In order to obtain a performance as good as a TA, the factors X, Y and Z are most important for our method. When X, Y, Z are at ...., then the performance is as good as a TA.
    \item By contrast, when we take the median on the same data, factors A, B and C are most important in determining its performance, and this is how: \textit{(show plots and explain dependencies)}
    \item When the number of weeks is lower than .../no ground truth our method should not be used, but in this and this case, our method is at least as good as real TA. Under these and these conditions, the median does worse than our method, and under these and these, median does better. This is an argument for using our method, because ........ \textit{(data's more likely to meet conditions for our method to work best)}
    \item ``as good as a TA'': here's how good a TA is from 3 offerings of data, aggregated. This is how well we should hope for our model to do, in order for it to successfully replace a TA.
    \item We don't evaluate Piech's model on synthetic data because we don't care what the important factors are for Piech (?). We also don't really want to make comparisons when we use two different data generating processes, because then it's difficult to compare the methods (?)
    % ^ maybe this isn't true, but that's what I think - Lena
\end{itemize}
% There's a lot of things we could potentially test. Maybe we should pare these down to the most useful/informative? I wrote down some of my thoughts - Lena
\textbf{Experiments to do:}

\begin{itemize}
    \item How accurate are the true grade predictions? 
    
    change the details of the generating process one at a time (default values are fit based on CPSC430 real data) and answer the following questions:
    % Heddy says look at all of these and see which ones are interesting, then select the ones that are and make a claim about them
    \begin{itemize}
        % I think number of students is an interesting thing to investigate, and relevant for people wanting to use our model - Lena
        \item How important is the number of students in class for predicting the true grades? (Plot num students vs  true grade estimates accuracy)\\
        \textit{Sample claim: our method does better than the median on larger classes, everything else kept constant (5 grades/week, 11 weeks, etc, this many calibrations, etc.).}
        % Grades per week is interesting to look at as well. Maybe a benchmark would be feedback from the course, if we have it (how many assignments is too much work for the students?) - Lena
        \item How important is the number of students per submission for predicting the true grades? (Plot num students per submission vs  true grade estimates accuracy)\\
        \textit{Sample claim: our method reaches TA-level requiring fewer grades/week than the median}
        % I think num weeks is less interesting to look at, because that's not something that classes that use MTA (including our offerings) can really change. - Lena
        \item How important is the number of weeks in class for predicting the true grades? (Plot num weeks vs  true grade estimates accuracy)\\
        \textit{Sample claim: ?}
        % I'm curious about the tradeoff between TA's and calibrations too, e.g. how many TA's are equivalent to how many calibrations for the same performance? - Lena
        \item How important is the number of TAs in class for predicting the true grades? (Plot num TAs vs  true grade estimates accuracy)\\
        \textit{Sample claim: our method needs this many fewer TA's (being distributed in the same way) than the median to do just as well.}
        % Calibrations are interesting to look at but I think it's also interesting to not include TA's at all and see what happens to the performance - Lena
        \item How important is the number of Calibrations in class for predicting the true grades? (Plot \#calibrations vs  true grade estimates accuracy)\textit{Sample claim: our method needs this many fewer calibrations than the median to do just as well.}
        % personally I think num. of calibrations is more interesting than number of TA's, because calibrations directly mean "amount of ground truth" whereas TA's are basically a noisy ground truth. Also, if we add TA's in at this stage, we have to decide in advance how we should allocate them, and make sure that's the best way to do it - Lena
        \item How important is the effort distribution in class for predicting the true grades?
        % Not sure what this means ^ - Lena
        \item How does our method compare with other methods (e.g. taking median, taking average, Piech's method) in terms of error (e.g, mean squared error)
        % keep dataset constant for each comparison, but generate many different datasets
        % how to generate same dataset and test Piech/our method on it? if we test on different datasets then we're not really comparing performance apples-to-apples I think - Lena
        \item How does our method compare with a real TA in terms of error (e.g, mean squared error)
     \end{itemize}
    \item How accurate are the estimated grader performances?
    % What's a good benchmark for estimating grader performances? TODO? Also, median can't estimate grader performances - Lena
    \begin{itemize}
        \item Repeat steps above but this time look at grader performances estimates 
    \end{itemize}
    \item How scalable our method is?
    % Should there be a benchmark for scalability? I think we should test scalability of Piech's method and our method, on real data. IDK about synthetic data - Lena
    % Not sure what the claim here is either, yet
    % Sample claim: memory/time usage does not become exponential with class size, and it's reasonably low (i.e. not days) for an average-sized class? - Lena
    \begin{itemize}
        \item What's the running time of the inference as a function of class size, number of weeks, and grades per submission?
        \item How much memory does it use as a function of class size, number of weeks, and grades per submission?
    \end{itemize}
    
\end{itemize}
 
  \subsection{Real world predictions}
\textbf{Question:} How does our method do on CPSC430 real data in terms of accuracy of estimates?
\begin{itemize}
    \item how did we tune up our hyperparameters (later (or maybe here?) do a sensitivity analysis on these hyperparameters)?
    \item How do we show that we've aggregated grades well?
    \begin{itemize}
        \item hide some observed TA grades and predict them by predicting the true grades; then calculate MSE. (note: we can use new calibrations and TA data and use that information in the paper) % not sure what this means "new calibrations and TA data" - Lena
        \item compare MSE to the median grade or mean or the random walk model vs random walk + censored data vs censored data
        % don't we also want to compare to Piech's method? - Lena
        \item claim that our method is as good as a TA even though a TA would not be great, e.g., calculate TA noise and try to be within a TA noise with inference. 
    \end{itemize}
    \item to show that we've estimated grader performances well
    \begin{itemize}
        \item  use TA spot checked reviews as true labels for effort draws and try to estimate those.
        \item Using Fall18/19 data, run the inference until week $n$ and compare dependability until week $n$ with what the TA said for that particular week's evaluation for a student that is spot checked.
    \end{itemize}
    \item How important is the choice of parameters in estimating true grades and dependabilites? Run sensitivity analysis
    % what is the sensitivity analysis for? what would be a possible claim here? - Lena
\end{itemize}


\subsection{Robustness to misspecification}
\textbf{Question:} Is our model more specified compared to Piech's model?
\begin{itemize}
    \item Step 1:
    \begin{itemize}
        \item Generate data using Piech model
        \item estimate true grades using Piech model and our model
        \item compare estimates
        \item claim that our model either does better or reasonably good on this data
    \end{itemize}
    \item Step 2:
    \begin{itemize}
        \item Generate data using our model
        \item estimate true grades using Piech model and our model
        \item compare estimations
        \item claim that Piech can not aggregate data generated by our model well
    \end{itemize}
\end{itemize}


\subsection{Robustness to student behavior (?)}
% low-effort student behaviour isn't something that a prof using our system can change... unless they use incentives, I guess - Lena

\begin{itemize}
    \item Plot a graph that compares MSE of different models when the number of low effort students decrease.

    \item Potentially a plot that has How many students do the bad behavior vs How much TA is needed
    \begin{itemize}
        \item Argue that if only a few are bad the inference detect this, if a lot of them are doing bad then the spot-checking system would take care of this.
    \end{itemize}

\end{itemize}
\subsection{Evaluate the effect of TAs and calibrations in the system (?)}
This is mostly plausible with synthetic data. 
\begin{itemize}
    \item spot check randomly
    \item spot check based on inference
    % Yeah I feel like maybe TA's should be left out of our experiments until this point... not sure - Lena
\end{itemize}

==> Better Peer Grading through Bayesian Inference (3)/old/inference.tex <==

% no longer closed form updates


\subsection{Technical details of the Bayesian inference method}
\begin{itemize}
    \item Describe the Gibbs sampling algorithm used in running the inference
\end{itemize}
(Refer to the Effort model theory doc.)


==> Better Peer Grading through Bayesian Inference (3)/old/model.tex <==
\gd{Preamble: recap what we're hoping to achieve with this model. It should capture integer-valued grades, low-effort grading behaviour, and grades with multiple components.}
In this section, we define the \emph{binary effort model} (BEM)...

\begin{figure}
    \centering
    \input{figures/model_bem}
    \caption{The BEM graphical model.}
    \label{fig:my_label}
\end{figure}

Following \citet{piech2013tuned}, we suppose that $U$ is a set of assignments and $V$ is a set of graders, consisting of both students and TAs. 
We write $v \to u$ to indicate that an assignment $u \in U$ was graded by a grader $v \in V$.
%The grading rubric consists of $C$ components, each of which can take on values in $\{0, 1,\dots, M\}$.
We consider the following set of latent and observable variables:

% describe variables 
% - true grades
% - reliabilities
% - efforts: clamp to 1 for TAs
% - effort draws
% - observed grades
% - reported grades: round to the nearest reportable value (ex: nearest integer)
\begin{itemize}
    \item \textbf{True grades:} For each assignment $u \in U$ and each rubric component $c \in \{1, \dots, C\}$, there is an underlying \emph{true grade} $s_{u,c} \in \mathbb{R}$.
    % \item \textbf{True grades:} Each assignment $u \in U$ has a vector of true grades $\bm{s}_u \in \mathbb{R}^C$, with separate true grades $\bm{s}_{u,c} \in \mathbb{R}$ for each rubric component $c \in \{1, \dots, C\}$. 
    %is the true grade for rubric component $c$.
    \item \textbf{Grader reliabilities}: Each grader $v \in V$ has a \emph{reliability} $\tau^v \in \mathbb{R}^+$ corresponding to their grading ability, with more reliable students tending to assign grades closer to the true grade. 
    \item \textbf{Grader efforts}: When grader $v$ grades an assignment $u$, they select an \emph{effort} $z_u^v \in \{0, 1\}$.
    If they put in \emph{high effort} ($z_u^v = 1$), they give a grade correlated with the assignment's true grade; if they put in \emph{low effort} ($z_u^v = 0$), they instead ignore the contents of the assignment, giving an uninformative grade (e.g., close to the class average).
    Each grader also has an \emph{effort probability} $e^v \in [0, 1]$, which is the probability that they put in high effort.
    % \item \textbf{Grader efforts}: Each grader $v \in V$ also has an \emph{effort} $e^v \in [0, 1]$, which is the probability that they give an informative grade to an assignment they are grading. 
    % When grading assignment $u$, they select an \emph{effort draw} $z_u^v \in \{0, 1\}$; they give an honest grade if this effort draw is $1$, but choose an uninformed grade independent of the assignment if the effort draw is $0$.
    \item \textbf{Observed grades}: When asked to grade assignment $u$, grader $v$ obtains an \emph{observed grade} $o_{u,c}^v \in \mathbb{R}$ for each rubric component $c \in \{1, \dots, C\}$ of the assignment.
    %, \dots, o_{u,C}^v
    \item \textbf{Reported grades}: Finally, graders use their observed grades to select integer-valued \emph{reported grades} $r_{u,c}^v \in \{0, 1, \dots, M\}$ from the rubric for each component $c \in \{1, \dots, C\}$ of assignment $u$.
\end{itemize}

% TAs and calibrations
We model TAs as graders who have a high (but unknown) reliability. % and always puts in high effort.
We also model calibrations as assignments which were graded by an ``instructor'' grader, who is known to have a very high reliability and always exerts high effort.

% describe BEM model
Specifically, we consider the following generating process:
\begin{alignat*}{2}
    \text{(True grades)}& \quad 
    s_{u,c} &&\sim \mathcal{N}(\mu_s, \tau_s) \\
    \text{(Reliabilities)}& \quad 
    \tau^v &&\sim \GammaDist(\alpha_\tau, \beta_\tau) \\
    \text{(Effort probabilities)}& \quad 
    e^v &&\sim \BetaDist(\alpha_e, \beta_e) \\
    \text{(Efforts)}& \quad
    z_u^v &&\sim \Ber(e^v) \\
    \text{(Observed grades)}& \quad
    o_{u,c}^v &&\sim \begin{cases}
        \mathcal{N}(s_{u,c}, \tau^v), & z_u^v = 1 \\
        \mathcal{N}(\mu_s, \tau_\ell), & z_u^v = 0 \\
    \end{cases} \\
    \text{(Reported grades)}& \quad
    r_{u,c}^v &&=  \begin{cases}
        M, & o_{u,c}^v > M \\
        \round(o_{u,c}^v), & o_u^v \in [0, M] \\
        0 , & o_{u,c}^v < 0 \\
    \end{cases} 
\end{alignat*}


% describe hyperparams
Here, $\mu_s$ and $\tau_s$ are the mean and precision of the true grade prior, $\alpha_\tau$ and $\beta_\tau$ parameterize the grader reliability prior, and $\alpha_e$ and $\beta_e$ parameterize the grader effort probability prior.
The low-effort grading behavior is to choose a grade close to the class average, plus Gaussian noise with precision $\tau_\ell$, and report its rounded value.
\gd{Support this with evidence from class and cite Hartline's scoring rule paper.}

% (figure: graphical model)
\begin{figure}
    \centering
    % \includegraphics{}
    TODO: graphical model?
    \caption{TODO: graphical model caption}
    \label{fig:model}
\end{figure}

% why not model bias?
% why model true grades as reals, not integers?
% What is the "reported grade" layer for? 
\gd{Explain some of our modeling choices here? No bias; real-valued true grades}

% two variants of the model
% - uncensored: treat grades as observed grades (as in Piech and most other work)
% - censored: treat grades as reported grades
Motivated by previous work, we consider one simplification of our model, where we remove reported grades from the model and instead treat the integer-valued reports as real-valued observed grades.
We refer to this variant as the \emph{uncensored BEM}.





% censored PG1
% - also consider similar modification to PG1

% first draft:
%In our model, each assignment $u$ has a \emph{true grade} $s_u \sim N(s_u; \mu_s, \tau_s)$, where $\mu_s$ is the class average and $\tau_s$ is the precision of the grades. Each student $v$ has a \emph{reliability} $\tau^v \sim \text{Gamma}(\tau^v; \alpha_\tau, \beta_\tau)$ and an \emph{effort} $e^v \in [0,1] \sim \text{Beta}(\alpha_e, \beta_e)$. Whenever student $v$ is asked to grade an assignment $u$, they decide an \emph{effort draw} $z_u^v \in \{0,1\} \sim \text{Ber}(e_u^v; e^v)$ . Then, they choose a \emph{reported grade} $r_u^v \sim P(r_u^v; o_u^v, z_u^v)$ based on the following:
%    \begin{itemize}
%        \item If $z_u^v = 1$ (``high effort''), they give $r_u^v = \text{round}(o_u^v)$, where $o_u^v \sim N(o_u^v; s_u, \tau^v)$ is their observed grade when they put in high effort. 
%        \item If $z_u^v = 0$ (``low effort''), they select $r_u^v \sim P_\ell(r_u^v)$ from a predetermined low-effort distribution. 
%    \end{itemize}

%We model TAs as highly reliable students who are always high effort. We also assume that we have set of calibrations for which true grades are known with high accuracy.  We'll also need two more pieces of notation. $I(r_u^v)$ denotes the \emph{interval} of observed grades that would round to the reported grade $r_u^v$. Typically, $I(r_u^v) = [r_u^v - \frac{1}{2}, r_u^v + \frac{1}{2}]$, but it's possible to use different interval sizes. Finally, the random variable $x \sim \text{truncnorm}(\mu, \tau, a, b)$ is drawn from a \emph{truncated normal} distribution with mean $\mu$ and precision $\tau$, subject to the bounds $a \le x \le b$. If $I = [a, b]$, $\text{truncnorm}(\mu, \tau, I)$ is shorthand for $\text{truncnorm}(\mu, \tau, a, b)$ (ie: $N(\mu, \tau)$ truncated to the interval $I$). 


==> Better Peer Grading through Bayesian Inference (3)/old/problem_statement.tex <==
\section{Details of the new grading mechanism}

\subsection{Students' Essay Grade}
\begin{itemize}
    \item After the deadline for submitting student reviews, run Bayesian inference on new and old data points gathered for each student. Use inference output as tentative essay grades.
    \item Once the TA grades are in (either true appeals or spot checks) finalize grades.
    \item Re-calculate them internally only for the sake of calculating more accurate grades for future weeks.
\end{itemize}

\subsection{Students' Weekly Peer Review Grade}
\begin{itemize}
    \item after the deadline for submitting student reviews, run Bayesian inference on new and old data points gathered from each student to calculated tentative effort and reliability estimates.
    \item Calculate the dependability score (this is yet to be defined formally) for each student.
    \item After TA grades are in, re-run inference and finalize dependability of each student for the week that they graded in. 
\end{itemize}

\subsection{Calibrations}
\begin{itemize}
    \item Once a new calibration is submitted:
    \begin{itemize}
        \item think of every other essay grade and dependability as observed except for the student who submitted the calibration
        \item run the inference to re-estimate dependability. 
    \end{itemize}
    \item This is fast because everything else is fixed. The result would mainly affect how student reviews are assigned. 
\end{itemize}


\subsection{Assigning student reviews}
\begin{itemize}
    \item Update beliefs about students' dependability by the essay submission deadline.
    \item Sort them based on that, match students with high dependability with each other.
    \item The exact matching algorithm is flexible. Probably the best way is to put them in a loop and have each student grade the next three students in the loop. 
\end{itemize}
  

\subsection{Assigning TA reviews}
A TA review or spot check consists of 
\begin{itemize}
    \item grading the essay carefully and updating its score.
    \item flagging each review either as high effort or low effort.
\end{itemize}
 The new true grade and information on student effort is then used to update dependability score for each student involved in the essay for that week. 
 
Spot checking budget is divided into three items:
\begin{itemize}
    \item High grades
    \item Random
    \item Submissions that are most likely appealed, e.g., high variance grades
\end{itemize}

\begin{figure*}
    \centering
    \includegraphics{figures/fall19-variance.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure*}

==> Better Peer Grading through Bayesian Inference (3)/outline.tex <==



Solving practical problems with using Bayesian inference in practice. 

discrete grades >> censoring >> maximizing the effect of censoring >> 

study what happens

reported class average

interpret grades

center your thought around the claim and what I can do to support that claim


EC outline (more incentives, less inference)

1 Intro (pitch):
- Main claim is about incentives
    ○ Effort model: inspired by Jason Hartline/Arpita Ghosh
    ○ Interpretability (MIP): a way of understanding the mechanism
    ○ Zombies: gives students a way to influence their rewards in a short time
    ○ TAs: inform spotchecking with confidence intervals (especially on dependability)
    ○ Censored data: helps with incentives of appealing (avoiding appeals to “round up” a grade)

1.1 Related work
- State of the art Bayesian inference models (PG1, Vancouver, GCN)
- Incentive problems in peer grading (from the EC community)
    - put here if talking English is fine
	
2 Bayesian modeling
2.1 Warmup: "standard" PG1 model
2.2 How we adjust it to make BEM
    - Effort
    - Censoring

3 Incentives 
% How the model helps with incentives when using it in a class:
    - Model features
        - Effort
        - Censoring
        - Grading graders
    - Zombies
    - MIP
    - spotchecks/appeals
    
4 Experiments
4.1 Synthetic data
- showing that we actually addressed them
    - true grade accuracy
    - recovering efforts/dependabilities
        - # calibrations/# TA grades, etc
        - Censored data in these too? 
        - (TA spotchecks?)
        - (ways of spotchecking?)
    - MIP doesn't ruin grades
        - Compare grades before and after MIP and show the changes
        - How to tune MIP parameters?
    - Zombies window size
        - show accuracy as a function of window size
    % - (student perceptions? anecdotes from 430?)
    
4.2 Real data
- evidence of the existence of low-effort behavior
    - students with less variance than final grade distribution

- assessing effectiveness of dependability scores
    - low variance graders have low effort, not for Piech [ those same people from above got caught ]
    - high variance graders are caught as unreliable
    - how good are TAs anyway? [Discussion: revisiting clamping efforts to 1?]

- show effectiveness of mixing with uniform?

- experimental setup:
    - where do hyper-parameters come from
    - ...













Introduction:

Peer grading is a wonderful thing
- helps students learn
    - more frequent and faster feedback
    - exposure to work at their own level of competence
    - internalization of the rubric
- helps manage large classes at lower cost

The AI community has recognized the design of peer grading systems as an important problem of interest.

There are two, somewhat interconnected strands of work in the literature:

1. statistical approaches (infer true grade, graders' reliabilities from students' joint reports)

2. peer prediction/mechanism design approaches (particular attention paid to the problem that students don't always have an incentive to report grades honestly; it's less work to do a superficial job grading)

3. of course, there are some lines of work that bring together both elements.

We start from a recent statistical approach and show how it can be advanced both to better model reality and to better reward good behavior and punish bad behavior, thereby bringing in many of the best ideas from the game theoretic literature.

In what follows, we begin by describing a statistical approach to inferring assignment grades and grader reliabilities that roughly follows Piech et al and captures the current state of the art (Section 2). We show how to elaborate this model in three key ways: (1) to perform (better/more reliably?) when grades are discrete instead of continuous; (2) to account for the fact that students may follow low-effort strategies that existing models would otherwise interpret as reliable grading; (3) to allow for the existence of TA graders (who always make an effort) and calibration assignments (whose true grades are already known) to improve the system's estimates of both true grades on student assignments and student reliabilities (Section 3). In Section 4 we explain why this architecture offers good incentives, particularly when combined with an appeal mechanism and TA spot checking. In Section 5 we present experimental data that shows the quantitative performance of our system. .....

---
Section 2: Existing state of the art

Piech model (whatever version of it we actually use).

Explained via a graphical picture.

How does inference work.

Maybe: some problems with it. Or, maybe give these in Sec 3 also
- rounded grades can show high agreement -> high reliabilities

---

Section 3: Methods

3.1 Censoring
  - model
  - inference
  - describe the inference problem this solves 

3.2 Low effort
  - model
  - uncensored inference
  - censored inference

3.3 TAs and calibrations

---

Section 4: Incentives

4.0 Do we want to talk about zumbies and MIP stuff here?

4.1 Grading graders

The core of an incentive scheme is to explicitly give students a grade for grading. How do we do this. Confidence interval; prior. Show that this score goes up with reliable grading, and also that students can improve their grade by doing more calibration.

4.2 Appeals

If someone gives another student a low grade, they will be reported. 

4.3 Spot checking

If someone gives another student a high grade, they might not be reported. Spot check these more. Also spot check other problematic cases; explain our various logic. Describe how TAs grade effort, but not reliability.

4.4 The problem of reporting the mean

Jason Hartline: students look pretty reliable when they report the mean.

Our solution: explicitly model this possibility, prior prefers it to effortful grading

Under our grading scheme described above, and with the mechanism where TAs observe effort (partly based on signals that live outside the model like the text of a review) this attack is no longer effective.

Arpita-style argument that no other attack is easy to carry out/focal?

----

Section 5: Synthetic data

    - scaling studies
        - how many samples does it take? How do you determine?
        - how is runtime as a function of class parameters? ("can I use this in my class?")

    - recovering inference parameters (as a function of class parameters)
        - what influences our ability to recover true grades?
            - scaling grades per assignment: BEM surpasses TA with 4 assignments; other methods need 6
            - TA grades: need ~1/3 of the class to be graded by TAs to match BEM's improvement
        - ...our ability to recover reliabilities/efforts?
            - scaling grades per student: more data per student helps censored BEM recover efforts
            - TA grades: adding a few TA grades helps recover reliabilities (makes sense they need to grade effort outside of the model)
            - calibrations: grading a few calibrations also helps with reliabilities and efforts

    - robustness to misspecification
        - wrong hyper-parameters (which ones matter?)
            - class average: getting low-effort distribution wrong makes a big impact on effort estimates
            - class grade variance: big impact on true grade estimates (why?); too small is bad for reliability estimates
            - reliability prior: extreme values ruin reliability and effort estimates, but generous range of good priors
            - effort prior: only affects effort estimates in uncensored BEM
            - low effort precision (needs correct range): too uniform makes everything worse; too concentrated makes uncensored BEM worse
        - wrong generating process (data from PG1)
            - over range of TA grades: (un)censored BEM recovers true grades and reliabilities as well as PG1
            - (grades per assignment: still running)
            - (stretch goal: how can it do this?)
        - how much of a difference does the censored model make? (stretch goal: okay to describe conceptually in section 3)
            - one lucky grade difference

----

Section 6: Real data

    - evidence of the existence of low-effort behavior
        - students with less variance than final grade distribution
    
    - show effectiveness of mixing with uniform?

    - experimental setup:
        - where do hyper-parameters come from
        - ...
 
    - assessing effectiveness of dependability scores
        - low variance graders have low effort, not for Piech [ those same people from above got caught ]
        - high variance graders are caught as unreliable
        - how good are TAs anyway? [Discussion: revisiting clamping efforts to 1?]

        
    
    






==> Better Peer Grading through Bayesian Inference (3)/real_data.tex <==
We now evaluate our contributions on real peer grading data, gathered between September 2018 and December 2021 from four offerings of an undergraduate-level computer science course on the ethical and societal impacts of computing. (Research use of this data was authorized by an ethics review board.)
In each offering of this course, approximately 120 students %between X and Y students 
wrote 11 weekly essays.
Each grade consisted of discrete values between 0 and 5 for each of four components (structure, evidence, subject matter and English). 
Overall, our experiments show that our model extensions (grader effort and censored observations) improved fit and that the explainable grades output by our MIP rarely differed from the (non-explainable) MAP estimates.

%\gd{Mention how we ran these classes. Maybe name them here if it makes that easier. Fall18/19 used a mechanism more like the peer prediction literature; Winter21 evaluated graders using a model with only efforts (I think); Fall21 added censoring.}
%\hz{add more details about class data in general. for example, how low effort grading looks like.}\klb{For that one I'd mention it in the place where we otherwise discuss low effort.}
% We begin by showing that the inference model that best explains our real data is one that models students' biases, efforts, and uses censoring (Section~\ref{sec: best_model}). Then, we look into different ablations of our best model to show the impact of each feature on the best model's estimations (Section~\ref{sec: ablations}). Finally, we show that using the true grades output from our MIP formulation produces virtually the same results as simply picking the grade with the largest posterior mass, showing that the MIP can improve grade interpretability at a negligible penalty to performance (Section~\ref{sec: MIP_stability_real}). 

Our experiments include data from three types of graders.
First, each student essay was graded by 4--5 peers, yielding between 6088 and 7068 peer grades per dataset. 
Second, each course was supported by a team of 3--5 TAs who spot checked between 474 and 644 essays, mostly in response to suspiciously high average grades, high disagreement between peer grades, and graders with poor historical performance. %TAs were well-trained and familiar with the grading rubric, so we model them as being well-calibrated, high-effort graders, with a reliability 2 to 3 times higher than a typical student, a bias of 0, and an 
Our TAs were diligent and responsible, so we clamped their efforts to 1 (i.e., their grades could never be explained away as coming from the low-effort distribution); we fit their bias and reliability parameters from data just as we did for students.
Third, each course included between 60 and 84 gold-standard ``calibration'' submissions that we used to train students; their grades were painstakingly agreed upon by the whole course staff in special grading sessions.
We model these grades as having being given by a special ``instructor'' grader, with efforts clamped to 1 and a reliability clamped to 16 (corresponding roughly to an 80\% accuracy of perfectly recovering true grades); we fit its bias parameter from data.

Ideally, we would evaluate our models based on their ability to recover assignments' true grades.
However, we lacked enough ground-truth values for a sound evaluation: while TAs and instructors are reliable sources of grades, they graded an unrepresentative sample of the submissions, and we did not have the resources to obtain TA grades more broadly after the classes were finished.
% \textcolor{red}{One could imagine evaluating our models based on their ability to recover the true values of the parameters (like true grades, reliabilities, etc) in the datasets. However, our real-world datasets did not include any ground-truth values for any parameters and we did not have the resources (e.g., TAs) to obtain them once these classes were finished.} %So we could not evaluate how accurately our models' posteriors recover these parameters' true values.}
Instead, we tested our models' ability to predict held out data---their \emph{held-out likelihood}~\cite{Vehtari2016}.
Running leave-one-out cross-validation would have been computationally prohibitive, given the size of our datasets and the cost of our inference procedure, so we instead used 10-fold stratified cross-validation.
We first split the dataset into 10 groups of $n/10$ peer grades, ensuring that no two peer grades on the same submission were in the same group.
Then, for each way of selecting 9 groups from the 10, we ran the model on these selected observations, summing the model's log likelihoods on the remaining group.
An exploratory experiment on one of our four datasets confirmed that this approach closely approximated leave-one-out cross-validation.
We use paired $t$-tests to make statistical comparisons between held-out likelihoods of several models on the same dataset.

Each time we fit our model to a dataset, we collected 4 runs of 1,100 Gibbs samples, discarding the first 100 burn-in samples from each run and concatenating the remainder; this took about 8 CPU hours.
We found that this number of samples made a good tradeoff between the runtime and sample complexity of our models: e.g., comparing to runs with 10,000 Gibbs samples, our protocol of gathering 4,000 samples caused an average error of 1\%, 3\%, and 1\%  on our estimates of true grades, reliabilities, and effort, respectively, and therefore had a small impact on our results.

%\subsection{Finding the Best Model}
%\label{sec: best_model}
In order to evaluate the effectiveness of our effort and censoring extensions to PG1, we compared models having both, one, or neither of these features.
We independently optimized each model's hyperparameters using randomized grid search, choosing the hyperparameters that maximized the model's held-out likelihood; full details of this hyperparameter search are presented in Appendix~\ref{sec: hyperparam_search}. 
We found that the model using both features had the highest held-out likelihood.
Furthermore, many of this model's hyperparameters had the same optimal values on all four classes, sharing the same true grade, % ($\mu_s = 4, \sigma_s= 0.8$), 
reliability, %($\alpha_\tau = \beta_\tau = 2$), 
and effort probability priors. % ($\alpha_e= 8, \beta_e = 2$).
They differed only (i)~in their bias priors, with two datasets giving rise to small biases ($\sigma_b = 0.1$) and two to larger biases ($\sigma_b = 1$); and (ii)~in their low-effort grading distributions, with low-effort reports being relatively diffuse in three datasets ($\tau_\ell = 1$) but more concentrated in the fourth ($\tau_\ell = 4$). 
% \subsection{Ablations on the best inference model.}

We then ran an ablation experiment, disabling each feature while holding the hyperparameters fixed.
We evaluated held-out likelihood of each ablated model along with the average absolute change in each student's grade. 
Our results, shown in Figure~\ref{fig:ablation}, indicate that both features improved the model's fit to data: removing censoring always caused significant drops in performance, while removing efforts had significant effects in the first two classes.
(The latter result is perhaps unsurprising: the later classes took greater lengths to disincentivize low-effort behavior, so detecting it is likely to have less impact on model performance.)
All model changes made small but meaningful changes to the final grades, averaging between 0.05 and 0.15 points on our 5-point scale, and seldom exceeding a single point change.

\begin{figure}
    \centering
    \includegraphics[trim={0 0.4cm 0 0}]{figures/real_data/ablation_final_1.pdf} 
    \caption{Model ablations. Each bar represents the change relative to the best-performing model, which included both censoring and biases for each dataset. Stars on log-likelihood bars show significance ($p < 0.05$).}
    \label{fig:ablation}
\end{figure}

Finally, we also investigated variations in model architecture beyond the two extensions introduced in this paper. First, we asked whether we could get good performance without bias terms. We could not; they helped substantially. Second, we asked whether PG5-style correlation between student's grades on their own submissions and their reliabilities was helpful. It was not, regardless of whether we included biases. Details of both experiments are given in Appendix~\ref{sec: ablations_appendix}.

%\subsection{Evaluating MIP Explanations}
%\label{sec: MIP_stability_real}
Having determined the superiority of our effort + censoring model, we used it to evaluate the extent to which the MIP had to deviate from submissions' MAP grades in order to present them as weighted averages of the graders' reports.
We set the MIP constants to the defaults recommended in Appendix~\ref{sec: mip}, allowing the graders' weights to change by at most $S=0.09$, with a minimum non-zero weight of $T=0.1$.
We found that replacing the MAP grades with the MIP's output would have caused only 3 to 6 percent of grades to change.%, showing that the MIP can improve grade interpretability at a negligible penalty to performance.

% \gd{Stretch goal: show that reliability/bias/effort confidence intervals are heterogeneous in early weeks, so asking students to calibrate based on uncertainty estimates would really have some bite.}


==> Better Peer Grading through Bayesian Inference (3)/related_work.tex <==
%Our methods draw from two lines of work in the peer grading literature: graphical models of peer grading, and the existence of strategic behavior in peer prediction systems.



%\paragraph{Alternative grade aggregation methods.}


%Notably, 
%\citet{fang2017rankwithta} propose an iterative method to estimate true grades, weighting an assignment's peer grade by the grading accuracy of each grader calcualted from the previous iteration. 
 %This work is similar to ours in that it uses input from TAs and instructors as a signal about students' performance. 

%Two recent closely related papers estimate grader biases and reliabilities an a way that seeks to strengthen the incentives offered to students~\citep{prajapati2020swagrader, chakraborty2018incentivizing}. The key idea is a ``social welfare score'' that measures the (beneficial or harmful) influence of a particular grader on the class. This work is similar to ours in the sense that it is based \cite{piech2013tuned} and is concerned with incentives, but we take a different approach to avoid low effort behavior in our system. 

% Main related work categories:


% \subsection{Probabilistic Modeling}
% The closest line of work to ours focuses on using probabilistic modeling, Bayesian inference, and machine learning to improve grading accuracy in peer grading systems. %~\cite{piech2013tuned,raman2014methods, shah2014some, labutov2017jag, sajjadi2016peer, kulkarni2014scaling, wang2019sspa, yuan2020practical, walsh2014peerrank,mi2015probabilistic, fang2017rankwithta, wang2019improving, namanloo2021improving}.
% The most influential work in this area is that of \citet{piech2013tuned}, which proposes three closely related graphical models for peer grading, termed PG1, PG2, and PG3. PG1 attributes a latent bias and reliability parameter to each student and a latent true grade to each assignment and estimates these parameters through Bayesian inference. The bias parameters specify the tendencies of individual students to be easy or hard graders; the reliability parameters model the inherent noise arising from each student's grading ability.  PG2 extends PG1 by assuming that the biases of students take a random walk as students do more grading. PG3 assumes that the reliabilities of students are correlated with their true grades. %\klb{move this}In our experiments with PG1 on our real class data, we observed it inferred very small bias terms overall. We think that this because early in the course, we ask students to grade a set of carefully graded calibration assignment, which would reduce any biases that they have. However, we have also observed that only modeling reliabilities does not explain some of the behaviors that we see in class. 

% % We use PG1 without biases as the base on our work because (1) we think that after students are calibrated in the system, the effect of biases (and their random walk) would be negligible and (2) we want the incentives for grading to be independent of assignment grades. %\hz{discuss bias here}%Overall, our model differs from PG1 in the following ways: (1) we take incentives or effort into account; (2) we do not include student biases in our model since we think that after students have gone through calibration mechanism, their biases would be significantly reduced; (3) our model handles the fact that students can only report inter-valued grades to the model. 
 
%  Inspired by~\citet{piech2013tuned}, various follow-up work focused on designing modified models to improve predictive accuracy. Notably, PG4 and PG5 extend PG3 by assuming that there is a probabilistic
% relation between graders reliabilities and their true grades, i.e., they assume that students with higher grades are better graders. PG6 and 7 extend PG4 and 5 by feeding the difference between grades into the their Bayesian network as well. 
 
%  %\citep{sajjadi2016peer,yuan2020practical,mi2015probabilistic,wang2019improving}. 

 
%  %. Their approach is similar to our work in the sense that it gives less weight to unreliable grading behavior. But, , 
 

% \subsection{Iterative approaches}

% There is a line of work in the literature that focuses on aggregating grades and incentiving high quality grading as point estimates using iterative approaches~cite(walsh and Vanvouver). In these approaches, the final grade of each assignment is set to be the weighted average of its reported grades, where the weight of each reported grades reflects the accuracy of the grader who submitted the grade. The grading accuracy for each grades reflect at each step reflects how far reported grades are from what the algorithms thinks about the true grade at each step. If TA grades are available these grades are always used at final true grades.  A nice property of such approaches is that they produce interpretable grades. However, they produce point estimates which does give much information about how confident the method is about each grades. They also do not handle discrete grades properly. 

% These approaches also suggest to use the estimates for grading accuracy as part of each students final grades so that students are encourage to put in the effort for grading better.

%  %For example, \citet{fang2017rankwithta} propose an iterative method to estimate true grades, weighting an assignment's peer grade by the grading accuracy of each grader calcualted from the previous iteration. 
%  %This work is similar to ours in that it uses input from TAs and instructors as a signal about students' performance. 
 
 
% % They explore two approaches regarding TAs: (1) where a TA is treated as a skillful student, and (2) where TA grades are used to estimate student biases before aggregation. Similarly, we model TAs as high reliability graders who always make an effort, leveraging this signal to obtain better estimates of the model's remaining parameters.
 
 
%  %\citet{raman2014methods} explores several probabilistic rank aggregation models and shows the efficacy of this type of grade aggregation compared to cardinal peer grading and traditional evaluation techniques. The main way in which their work differs from ours is that it uses peer grades in an ordinal, rather than cardinal, form. However, the overall objective of accurate peer grade aggregation aligns with our own.

% % Peer prediction approaches

% % 




% % There are two interconnected strands of work in the literature that closely relate to our work: mechanism design approaches, which focus on the problem that students do not always have the incentive to put in high effort to grade their peers accurately; and statistical approaches, which focus on inferring true grades and graders' reliabilities based on students' grading behavior.

% \subsection{Incentives and modeling student effort}

% There is a prominent line of work in the mechanism design literature focusing on incentivizing high quality grading in environments such as peer grading and reviewing~\citep{liu2018surrogate,goel2019deep, faltings2012eliciting,prelec2004bayesian,radanovic2014incentives,riley2014minimum,witkowski2012robust,witkowski2013dwelling,jurca2009mechanisms,kong2016putting,jurca2005enforcing,kamble2015truth,radanovic2013robust,shnayder2016informed, gao2019incentivizing,zarkoob2020report}.
% Work in this area is mostly centered around the idea of peer prediction.
% In such mechanisms, students (agents) are incentivized to behave honestly based on how their behavior compares to their classmates. 
% A common issue associated with most peer prediction mechanisms is that they rise to uninformative equilibria in which students would prefer to game the system by reporting uninformative grades~\citep{jurca2009mechanisms,witkowski2013dwelling,kong2016putting,shnayder2016informed,dasgupta2013crowdsourced,gao2019incentivizing,zarkoob2020report}. 
% Much of the work in the peer prediction literature focuses on using mechanism design and statistical methods to obtain incentive mechanisms that do not suffer from uninformative equilibria~\citep{liu2018surrogate,goel2019deep}. 
% While such attempts are mostly orthogonal to this work, modeling low-effort behavior in our models is partly motivated by the existence of uninformative behavior by students in a peer grading environment.

% %\gd{Too much detail?}

% \subsection{Other closely related work}

% Recent work by \citet{burrell2021measurement} discusses the importance of measuring effort in peer grading settings and focuses on the question of how to grade the graders. In their model of peer grading, grades are discrete and effort is defined as the number of draws that each grader obtains from a latent binomial distribution that is specified by the grader bias and the true grade distribution. %They also look into PG1~\gd{We haven't said what this is yet.} as the continues version of their model and consider reliability as the equivalent to their effort level. 
% They experiment with using a variety of out-of-the-box peer prediction mechanisms to reward graders, finding that these peer prediction reward functions do not accurately reflect grader effort levels. 
% %(or reliability in the case of PG1) used to generate the data. 
% In contrast, we use a simpler model of grader effort in which graders make binary effort decisions.
% We treat discrete-valued grades as censored data, allowing us to perform inference on them, and focus on our models' abilities to correctly aggregate true grades. 
% % Our work uses a similar model of grader effort, 
% % Their model of effort is different from ours and is not applicable to our setting. Also, they are not at all concerned with aggregating reported grades to estimate true grades. %In contrast, we start from PG1 and explicitly integrate efforts into it. This helps us to estimate true grades better in the presence of such low effort behavior and also gives us a reliable way to grade the graders.
% % Also, we handle discrete grades by thinking about reported grades as censored data. 
 

 
% Finally, two recent papers extend \citet{piech2013tuned}'s PG1 model to estimate grader biases and reliabilities an a way that seeks to strengthen the incentives offered to students~\citep{prajapati2020swagrader, chakraborty2018incentivizing}. The key idea is a ``social welfare score'' that measures the (beneficial or harmful) influence of a particular grader on the class. This work is similar to ours in the sense that it extends \cite{piech2013tuned} and is concerned with incentives, but we take a different approach to avoid low effort behavior in our system. We do not see how its incentive properties could be tested without deploying it in practice, which we did not do, and so we do not evaluate it in this paper.


% \subsection{Ordinal approaches}

% There is a line of work that does peer grading in a world where graders are asked to compare the submissions that they are assigned to grade and give an ordering over them~\cite{shah2013case,mi2015probabilistic,raman2014methods}. These partial orderings are then merged to obtain a total ordering over all the submissions and is used to assign final grades to students' submissions. The work in this area argues that ordinal approaches work better in practice because it is easier for students to compare submissions and say which ones better that the other rather than assigning a raw numerical value to their quality. However, \cite{de2014crowdgrader} mentions that students reported uneasiness to rate their peers. Furthermore, we believe that the presence of calibration assignments should make easy the concerns over having students assigning numerical grades to their peers. 


%~\citet{lu2015grading} studies look into whether the following factors incentivize students to make an effort during peer grading: (1) knowledge that you are being graded, and/or (2) the opportunity to evaluate other students' peer grading. The position was taken that it seemed counterproductive to reward or punish good grading since students are simply there to learn the material, not to learn to grade. It was found that when students were shown evidence that their peers are producing high-quality grading, then this motivates them to do the same. This paper, by comparison to our work, examines incentives rather than peer grade aggregation and presents a novel view of them.


 
% - Papers that implement various peer grading systems
 
% \textit{ComPAIR: A New Online Tool Using Adaptive
% Comparative Judgement to Support Learning with Peer
% Feedback} ~\cite{potter2017compair} -- In this paper's experiment, students are shown increasingly similar assignments from their peers and asked to rank them along several dimensions. Results show perceived learning benefits of the system. No focus is given to crowdsourcing, grade aggregation, or training students to grade better. The clearest difference between this study and our work is the paper's focus on student experience rather than peer grade aggregation.
 
 
 
 
 
 
 %This procedure is compared to PeerRank ~\cite{walsh2014peerrank} using tests on synthetic data, and while both methods perform far better than aggregation using the average, RankwithTA outperforms PeerRank slightly.


% In~\citep{wang2019sspa} grade aggregation of peer grades is done using similarity measures of peers to each other, and to the instructor. This work is similar to our work in that it assigns to each assignment a weighted average of the graders' reports. However, the weight for each grader is computed to be a similarity measure (between 0 and 1) between this grader and a TA or instructor. This paper shows on Sajjadi's dataset ~\cite{sajjadi2016peer} an improvement to using the average for grade aggregation.
 
%  \begin{itemize}
%  \item \textit{Tuned Models of Peer Assessment in MOOCs} ~\cite{piech2013tuned} -- Piech
 
%   \item \textit{Methods for Ordinal Peer Grading} ~\cite{raman2014methods} -- This paper gets students in MOOCs to perform comparisons (ordinal peer grading) as opposed to absolute rankings of assignments, since it is shown to be easier to do. They also explore several probabilistic rank aggregation models, and show the efficacy of this type of grade aggregation compared to cardinal peer grading and traditional evaluation techniques. The main way in which this work differs from ours is that it uses peer grades in an ordinal, rather than cardinal, form. The overall objective of accurate peer grade aggregation aligns with our own.
 
 
%  \item \textit{Some Scaling Laws for MOOC Assessments} ~\cite{shah2014some} -- As class size increases, a theorem is posited that fixed proportion of students will make grading errors. This paper uses dimensionality reduction and clustering to allow the fraction of errors to go to zero as the class size grows. In effect, a grade aggregation technique via clustering can be used to prevent assignments from being given final grades that are incorrect. This technique is introduced theoretically, but not tested empirically, but both this work and ours is focused on improving the accuracy of peer grade aggregation methods.

% \item \textit{JAG: A Crowdsourcing Framework
% for Joint Assessment and Peer Grading} ~\cite{labutov2017jag} -- this paper frames peer grading as the answering of multiple-choice questions (MCQs) for which the answer key is not known, with two possible answers for each question. They construct a probabilistic model with student ability and question difficulty, which is then fit using EM. This model does not take into account incentives or effort, since they assume that a (relatively) low-ability student will simply guess an answer to each MCQ. This model is not suitable for our use, since assignment grades that are real values may admit grading strategies that would not make sense for a multiple choice test. Furthermore, this model differs from ours in that it only admits two possible answers for each MCQ.

% \item \textit{Peer Grading in a Course on Algorithms and Data Structures:Machine Learning Algorithms do not Improve over Simple Baselines} ~\cite{sajjadi2016peer} -- in a computer science class, a probabilistic model based on~\cite{piech2013tuned} was used to predict the true grades of assignments, and compared to several other aggregation methods. TA's were taken as ground truth, and it was found that taking the mean did not improve over using~\cite{piech2013tuned}'s probabilistic model. This paper's did not propose or test an effort-based model. In comparing ordinal ranking algorithms and the bias-reliability model, it was found that in almost all cases, both algorithms performed worse than simply taking the mean. One of the likely reasons for this is the nature of grading error -- it was very easy for students to miss a single error in a question while marking, and give a substantially higher mark than deserved. As we are testing on essays, it is possible that grading error will be more adherent to model assumptions in our case.

% \item \textit{Scaling Short-answer Grading by Combining Peer
% Assessment with Algorithmic Scoring} ~\cite{kulkarni2014scaling} -- instead of aggregating peer grades, an algorithm first determines how many peer graders to assign to an assignment. Then, based on how much  agreement there is between these peers, the mechanism may add more peers to grade the assignment. This method was shown to perform better than using the median for grade aggregation. This method is quite different from ours in that it uses NLP to direct the amount of peer assessments an assignment gets. It assumes simple answers to the assignments, either binary answers or enumerative short answers. Its method of aggregation is based on several peers independently reaching the same consensus in their marking.

% \item \textit{Practical Methods for Semi-automated Peer Grading
% in a Classroom Setting} ~\cite{yuan2020practical} -- This paper builds upon Piech and other peer grade aggregation mechanisms by using the idea of bias. However, instead of estimating it using Gibbs sampling from a probabilistic model, bias is estimated only from calibrations. Finally, the quality of reviews is estimated from the content of the review itself; this review quality is then used to give some reviews more or less influence on the final grade. Several methods are used to estimate the quality of reviews: review length as well as language models. This work is very similar to ours, but neglects to take into account the possibility of low-effort behaviour in students, whether through an explicit model, or through incentives.

% \item \textit{The PeerRank Method for Peer Assessment} ~\cite{walsh2014peerrank} -- This method uses an iterative procedure similar to PageRank to estimate grader reliability. It is very similar to the PG3 model that Piech describes in their paper. This approach ties the grade that a paper gets to the ability of the grader, which creates an incentive for each grader to grade as accurately as possible. The PeerRank method outperforms the average in experiments on synthetic data. We do not believe that both the grade a student obtains and this student's grading ability should be represented by one value, so we do not take the approach investigated by this paper.

% \item \textit{Human-machine hybrid peer grading in
% SPOCs} ~\cite{han2020human} -- This paper argues that Bayesian models such as those developed by Piech perform worse on small classes (SPOCs) than on MOOCs. For smaller classes, random or unreliable grading behaviour is more of a problem during grade aggregation. Methods are proposed in order to filter the peer grades before applying grade aggregation frameworks to them. These methods range from naive Bayes to CNN's, and use the text itself to assign a score to the assignment. The system then discards any peer grade that is further from this score than a predefined threshold. When tested on a real class and compared with other probabilistic models, this paper's method acheives a much lower RMSE. This work is different from ours in that it integrates automated grading into the system, and does not innovate on the probabilistic model, but our idea of identifying low-effort students and letting them have less influence on the final grade is similarly motivated.

% \item \textit{Probabilistic Graphical Models for Boosting
% Cardinal and Ordinal Peer Grading in MOOCs} ~\cite{mi2015probabilistic} -- This work extends Piech's work via new, related models called PG4 and PG5. They expand on Piech's PG3 model, where a student's reliability is a deterministic linear function of the true grade a student got. However, they do not believe that this function is truly linear, or that it is deterministic. This work reintroduces reliability as a random variable, but explores variations on the distribution it comes from. PG4 sets the reliability as being sampled from the Gamma distribution, with shape determined by the true grade. PG5 sets the reliability to be sampled from a normal centered at the true grade. PG4 and PG5 perform better than the original PG1-3 on a dataset with approximately 7 thousand peer grades. This paper also compares the aggregation of cardinal and ordinal peer grades. The approach taken in this work is very similar to ours, but we do not believe that linking peer grading ability and score on an assignment would accurately reflect the score the assignment should obtain. Moreover, the problem of explicitly capturing effort (or incentivizing it) is not within the scope of the paper.

% \item \textit{Improving Peer Assessment Accuracy by Incorporating
% Relative Peer Grades} ~\cite{wang2019improving} -- This work is motivated by the observation that relative peer grades (the difference in peer grades given by one student to two different assignments) are robust to that student's bias. The authors extended PG1-3 of Piech's work to account for relative peer grades in three more probabilistic models. It was found that by RMSE measures, these new models outperformed Piech's three models. This work is similar to our work in its approach, but there is still the question of why relative peer grades are not already   implicitly accounted for in Piech's models. Also, this work does not concern itself with effort models or incentives.


%  \end{itemize}
 




==> Better Peer Grading through Bayesian Inference (3)/synthetic_data.tex <==
% preamble
While our experiments on real class data allowed us to test how well our models described real peer-grading behavior, they gave us no way to check the accuracy of the parameter estimates.
Of course, giving accurate grades (either for submissions or students' grading abilities) is a primary focus of peer grading systems.
We therefore conducted further experiments on \emph{synthetic} data, generating parameters and reported grades according to our best-fitting models from the previous section, and evaluating how well the posteriors recovered the latent parameters' true values.
This methodology allowed us to test how our estimates improved as the amount of grading data increased, how sensitive they were to the choice of hyperparameters, and whether explaining grades with our MIP increased their error.

The previous section showed that a model incorporating both efforts and censoring had the best performance on all four datasets, but its optimal hyperparameters varied, with only two datasets having exactly the same optimal hyperparameters.
Thus, we show results here based on one representative dataset, with full results for all three sets of optimal hyperparameters in Appendix~\ref{sec: parameter_recovery_appnedix} and~\ref{sec: misspec_appendix}. 
Unless otherwise specified, we simulated courses consisting of 10 weeks, with 120 students each making 1 submission and grading 4 peers' submissions each week.
The grading rubric had four components, each of which was given an integer grade between 0 to 5.
We also included 3 TAs who grade 25\% of submissions; we clamped their effort parameters to 1. We simulated TAs as being more reliable than most students: inspired by our real data, we gave TAs a mean reliability of 2 and gave students' mean reliability of 1.

We evaluated true grade and bias estimates via \emph{Mean Absolute Error (MAE)}. We also computed accuracy (the fraction of true grade MAP estimates equal to the rounded true grade) and RMSE, finding qualitatively similar conclusions with these measures.
%In our accuracy calculations, we use the MAP estimates of the true grades.
%\gd{mention that we're testing max-likelihood estimates of true grades.}
We found that some models produced inaccurate reliability and effort estimates, but judged that this was less important because rewarding good grading only requires students to be \textit{ranked} in the correct order. Accordingly, we evaluated our reliability and effort estimates with the Spearman rank-order correlation coefficient, measuring how similarly students were ranked by the estimates and true values.
In each case, we report the mean and 95\% confidence intervals of each metric across inference runs on 15 simulated datasets.
We also compare our true grade MAEs to a hypothetical TA with a reliability of 2 (who achieves a mean absolute error of 0.48), allowing us to ask how much data is required to effectively substitute for a TA.

\subsection{Parameter Recovery}
\label{sec:parameter_recovery}
We begin by testing how the model's parameter estimates were affected by the amount of grading data available.
One obvious way to control the amount of data is to change the number of students in the simulated class. However, this change had surprisingly little impact on the inference problem's difficulty, because as the class size varies, each grader continued to grade a total of 40 submissions, and each submission continued to receive 4 grades.
Instead, we control these two dimensions separately, independently varying the number of grades from each student and the number of grades given to each submission. %, showing how each of these changes affect parameter estimates. 

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.75\linewidth,trim={0 0.4cm 0 0}]{figures/synthetic/consistency_final_2.pdf} 
    \includegraphics[scale=0.75,trim={0 0.4cm 0 0}]{figures/misspec_params/misspec_final_2.pdf}
    \caption{Effects of varying dataset size on (a) reliabilities; (b) effort probabilities; (c) true grades. Robustness of model outputs to misspecified hyperparameters: true grade (d) average and (e) stdev; (f) low-effort precision; (g) bias stdev.}
    \label{fig: consistency}
    \label{fig: misspec}
\end{figure*}

\paragraph{Varying grades per grader.}
First, we changed the number of grades given by each student by varying the number of weeks in the class.
Here, each assignment always received 4 grades, but the number of grades from each student scaled linearly with the number of weeks.
The results (Figure~\ref{fig: consistency}a-b) show that increasing the size of the dataset in this way improved grader quality estimates.
Reliability estimates had an appreciable correlation of 0.6 after just one week of data, improving substantially to 0.9 after 8 weeks.
Effort estimates followed a similar trend, but were much more difficult to estimate: one week of data produced a much poorer correlation of 0.3, with later weeks improving to 0.7.
Bias estimates, given in the appendix, also improved with additional data.

Perhaps surprisingly, true grade estimates improved very little as the number of weeks grew.
This suggests that, with only 4 grades per submission, most of the inaccuracy in the model's true grade estimates was driven by aggregating a small number of noisy signals, rather than because estimates of graders' reliabilities, biases, and efforts were inaccurate.

\paragraph{Varying grades per submission.} 
Next, we changed the number of graders in each course, holding the number of weekly submissions fixed at 40 and each student's grading workload at 4 grades per week. 
Adding graders in this way increased the number of grades given to each submission but preserved the amount of data about each grader, isolating the effect of additional information on each assignment. 
The impact of this change on true grade recovery is shown in Figure~\ref{fig: consistency}c.
These results indicate that adding additional peer graders on each submission substantially reduced true grade MAE, from 0.52 with a single grader to 0.41 with four---well below the MAE of a TA.
Adding more graders decreased true grade MAEs far lower, reaching below 0.2 with 32 graders. % converging to 100\% accuracy would take an enormous amount of grading effort.

Increasing the amount of data in this way had little effect on the model's ability to recover students' reliabilities, biases, and effort probabilities.
This suggests that error in those estimates was driven primarily by noise in the reported grades, not by noise in the underlying true grade estimates.
% Further, these inaccuracies are the likely cause for the slow convergence rate of true grade accuracies.

% \begin{figure}[t]
%     \includegraphics[scale=0.55]{figures/synthetic/effort_relaiblity_consistancy.pdf} 
%     \caption{Reliability consistency}
%     \label{fig: effort_reliablity_consistency}
% \end{figure}

% \begin{figure*}
%     \centering
%     \begin{tabular}{cc}
%         \includegraphics{figures/synthetic/grades_per_student_reliabilities.png} &
%         \includegraphics{figures/synthetic/grades_per_student_efforts.png} \\
%          (a) & (b)
%     \end{tabular}
%     \caption{Reliability and effort recovery, changing number of grades from each student}
%     \label{fig:recovery_grades_per_student_reliabilities}
% \end{figure*}


\subsection{Robustness to Incorrect Hyperparameters}
\label{sec:synthetic_robustness}
While the synthetic experiments we have discussed so far show that we were able to recover the model's parameters with sufficient data, they assumed knowledge of the hyperparameters used to generate this data.
%In practice, users of this system do not know the true settings of each of the hyperparameters.
We now ask whether it is crucial to set these hyperparameters correctly, or whether the model still robustly recovers parameters of interest when given different hyperparameter settings than those used to generate the data.
%To answer this question, we ran a misspecification experiment, simulating data from the same generating distribution, but running inference with hyperparameters that were set incorrectly. 
We tested our models under seven changes to the hyperparameters, varying the true grade mean $\mu_s$; the true grade standard deviation $\sigma_s$; the bias standard deviation $\sigma_b$; the reliability prior mean $\alpha_\tau / \beta_\tau$; the reliability prior variance $\alpha_\tau / \beta_\tau^2$; the effort probability mean $\alpha_e / \beta_e$; and the low-effort precision $\tau_\ell$. 

% In this section, we study the robustness of our model to misspecification of the data generating process through setting the hyperparameters incorrectly. We perform these experiments on generated datasets with 120 students submitting 1 assignment and grading 5 others (4 peers, 1 calibration) each week.
% Additionally, a single TA spot checks a random 25\% of the submissions each week. 

Overall, we found that many of these changes to the hyperparameters had small and statistically insignificant effects on the inference results; these complete results are shown in Appendix~\ref{sec: misspec_appendix}.
Notably, we found that the model's performance was quite robust to changes in the reliability and effort probability priors. We show four exceptions in Figure~\ref{fig: misspec}: using an incorrect mean or standard deviation for the true grade prior substantially increased true grade MAE from 0.44 to as high as 0.53; incorrectly specifying the low effort distribution $\tau_\ell$ was very detrimental to the effort probability estimates; and using a bias prior with a standard deviation far below its true value hurt bias estimates.



\subsection{MIP stability}

Lastly, we tested the impact of assigning grades based on explanations from our MIP formulation, rather than our model's MAP estimates of true grades, as we varied the number of peer grades given to each submission.
The results are shown in Figure~\ref{fig: mip_stability_synthetic}.
With only a single grader, the MIP output was equal to the mean of the Gibbs samples, which is much less accurate than the MAP. 
However, with additional graders, the MIP gained the flexibility to recover MAP grades, reaching nearly equal MAEs at 7 graders per submission.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth,trim={0 0.5cm 0 0}]{figures/synthetic/mip_stability_synthetic_final_3.pdf} 
    \caption{Effect of MIP explanations on true grade MAE.}
    \label{fig: mip_stability_synthetic}
\end{figure}

% \gd{Stretch goal: compare reliability CIs to reliability errors}

==> figures/model_bem.tex <==
\tikz{
    \node[obs] (observed_grade) {$o_{u,c}^v$};
    \node[obs, dashed, below=0.6 of observed_grade] (reported_grade) {$r_{u,c}^v$};
    
    \node[latent,above=0.6 of observed_grade,xshift=-1.5cm] (true_grade) {$s_{u,c}$}; 
    \node[const, above=1.2 of true_grade, xshift=-0.3cm] (mu_s) {$\mu_s$}; 
    \node[const, above=1.2 of true_grade, xshift= 0.3cm] (sigma_s) {$\tau_s$};
    
    \node[latent,above=0.6 of observed_grade,xshift= 1.7cm] (effort) {$z_u^v$};
    \node[latent,above=0.8 of effort,xshift= 0cm] (effort_prob) {$e^v$};
    \node[const,above=0.8of effort_prob,xshift=-0.3cm] (alpha_e) {$\alpha_e$};
    \node[const,above=0.8of effort_prob,xshift= 0.3cm] (beta_e) {$\beta_e$};
    
    \node[latent,left=2 of effort_prob,xshift= 1cm] (reliability) {$\tau^v$};
    \node[const,above=0.8 of reliability,xshift=-0.3cm] (alpha_tau) {$\alpha_\tau$};
    \node[const,above=0.8 of reliability,xshift= 0.3cm] (beta_tau) {$\beta_\tau$};
    
    \node[const, left=2.5of observed_grade, yshift=1.0cm] (tau_l) {$\tau_\ell$};
    % plate
    % \plate [inner sep=.3cm,xshift=.02cm,yshift=.2cm] {assignment_plate} {(true_grade)} {\begin{tabular}{l}assignments $u$ \\ components $c$\end{tabular}};
    % \plate [inner sep=.3cm,xshift=.02cm,yshift=.2cm] {student_plate} {(reliability)(effort_prob)} {graders $v$};
    \plate [inner sep=.3cm] {c} {(true_grade)(observed_grade)(reported_grade)} {$c$};
    \plate [inner sep=.3cm] {u} {(true_grade)(observed_grade)(reported_grade)(effort)(c.north west)(c.south west)} {$u$};
    \plate [inner sep=.3cm] {v} {(reliability)(effort_prob)(effort)(observed_grade)(reported_grade)(u.south east)} {$v$};
    % edges
    \edge {mu_s, sigma_s} {true_grade}
    \edge {alpha_tau, beta_tau} {reliability}
    \edge {effort_prob} {effort}
    \edge {alpha_e, beta_e} {effort_prob}
    \edge {true_grade, reliability, effort, tau_l} {observed_grade}
    \edge {observed_grade} {reported_grade}
}



==> figures/model_pg1.tex <==
\tikz{
    \node[obs] (observed_grade) {$o_{u,c}^v$};
    \node[obs, dashed, below=0.6 of observed_grade] (reported_grade) {$r_{u,c}^v$};
    
    \node[latent,above=0.6 of observed_grade,xshift=-1.2cm] (true_grade) {$s_{u,c}$}; 
    \node[const, above=0.8 of true_grade, xshift=-0.3cm] (mu_s) {$\mu_s$}; 
    \node[const, above=0.8 of true_grade, xshift= 0.3cm] (sigma_s) {$\sigma_s$};
    
    \node[latent,above=0.6 of observed_grade,xshift= 1.2cm] (reliability) {$\tau^v$};
    \node[const,above=0.8 of reliability,xshift=-0.3cm] (alpha_tau) {$\alpha_\tau$};
    \node[const,above=0.8 of reliability,xshift= 0.3cm] (beta_tau) {$\beta_\tau$};
    
    \node[latent,above=0.6 of observed_grade,xshift= 2.5cm] (bias) {$b^v$};
    \node[const,above=0.8 of bias,xshift=-0.3cm] (mu_b) {$\mu_b$};
    \node[const,above=0.8 of bias,xshift= 0.3cm] (sigma_b) {$\sigma_b$};
    % plate
    % \plate [inner sep=.3cm,xshift=.02cm,yshift=.2cm] {assignment_plate} {(true_grade)} {\begin{tabular}{l}assignments $u$ \\ components $c$\end{tabular}};
    % \plate [inner sep=.3cm,xshift=.02cm,yshift=.2cm] {student_plate} {(reliability)(bias)} {graders $v$};
    % alternative plates: include observed grade?
    \plate [inner sep=0.3cm] {assignment_plate} {(true_grade)(observed_grade)(reported_grade)} {$u$, $c$}
    \plate [inner sep=0.2cm] {student_plate} {(reliability)(bias)(observed_grade)(reported_grade)(assignment_plate.south east)(assignment_plate.north east)} {$v$}
    
    % \plate [inner sep=.3cm,xshift=.02cm,yshift=.2cm] {assignment_plate} {(observed_grade)(true_grade)} {\begin{tabular}{l}assignment $u$ \\ component $c$\end{tabular}};
    % \plate [inner sep=.3cm,xshift=.02cm,yshift=.2cm] {student_plate} {(observed_grade)(reliability)(bias)} {grader $v$};
    % edges
    \edge {mu_s, sigma_s} {true_grade}
    \edge {alpha_tau, beta_tau} {reliability}
    \edge {mu_b, sigma_b} {bias}
    \edge {true_grade, reliability, bias} {observed_grade}
    \edge {observed_grade} {reported_grade}
}



==> old/evals.tex <==
\textbf{Question:} What kind of evaluations are needed to convince ourselves and others that the Bayesian inference method is a reliable tool to use in a real course. 

% Note: we might actually want to evaluate our inference WITHOUT TA's separately from TA's effect (or optimal spotchecking methods) - Lena

\subsection{Synthetic data experiments}

\textbf{Question:} How accurate are the estimates of true grades and dependabilities using synthetic data in a CPSC430 like environment (~100 students and 4 grades per assignment)? what are the driving factor\\

\textbf{Sample Answer:} 
\begin{itemize}
    \item In order to obtain a performance as good as a TA, the factors X, Y and Z are most important for our method. When X, Y, Z are at ...., then the performance is as good as a TA.
    \item By contrast, when we take the median on the same data, factors A, B and C are most important in determining its performance, and this is how: \textit{(show plots and explain dependencies)}
    \item When the number of weeks is lower than .../no ground truth our method should not be used, but in this and this case, our method is at least as good as real TA. Under these and these conditions, the median does worse than our method, and under these and these, median does better. This is an argument for using our method, because ........ \textit{(data's more likely to meet conditions for our method to work best)}
    \item ``as good as a TA'': here's how good a TA is from 3 offerings of data, aggregated. This is how well we should hope for our model to do, in order for it to successfully replace a TA.
    \item We don't evaluate Piech's model on synthetic data because we don't care what the important factors are for Piech (?). We also don't really want to make comparisons when we use two different data generating processes, because then it's difficult to compare the methods (?)
    % ^ maybe this isn't true, but that's what I think - Lena
\end{itemize}
% There's a lot of things we could potentially test. Maybe we should pare these down to the most useful/informative? I wrote down some of my thoughts - Lena
\textbf{Experiments to do:}

\begin{itemize}
    \item How accurate are the true grade predictions? 
    
    change the details of the generating process one at a time (default values are fit based on CPSC430 real data) and answer the following questions:
    % Heddy says look at all of these and see which ones are interesting, then select the ones that are and make a claim about them
    \begin{itemize}
        % I think number of students is an interesting thing to investigate, and relevant for people wanting to use our model - Lena
        \item How important is the number of students in class for predicting the true grades? (Plot num students vs  true grade estimates accuracy)\\
        \textit{Sample claim: our method does better than the median on larger classes, everything else kept constant (5 grades/week, 11 weeks, etc, this many calibrations, etc.).}
        % Grades per week is interesting to look at as well. Maybe a benchmark would be feedback from the course, if we have it (how many assignments is too much work for the students?) - Lena
        \item How important is the number of students per submission for predicting the true grades? (Plot num students per submission vs  true grade estimates accuracy)\\
        \textit{Sample claim: our method reaches TA-level requiring fewer grades/week than the median}
        % I think num weeks is less interesting to look at, because that's not something that classes that use MTA (including our offerings) can really change. - Lena
        \item How important is the number of weeks in class for predicting the true grades? (Plot num weeks vs  true grade estimates accuracy)\\
        \textit{Sample claim: ?}
        % I'm curious about the tradeoff between TA's and calibrations too, e.g. how many TA's are equivalent to how many calibrations for the same performance? - Lena
        \item How important is the number of TAs in class for predicting the true grades? (Plot num TAs vs  true grade estimates accuracy)\\
        \textit{Sample claim: our method needs this many fewer TA's (being distributed in the same way) than the median to do just as well.}
        % Calibrations are interesting to look at but I think it's also interesting to not include TA's at all and see what happens to the performance - Lena
        \item How important is the number of Calibrations in class for predicting the true grades? (Plot \#calibrations vs  true grade estimates accuracy)\textit{Sample claim: our method needs this many fewer calibrations than the median to do just as well.}
        % personally I think num. of calibrations is more interesting than number of TA's, because calibrations directly mean "amount of ground truth" whereas TA's are basically a noisy ground truth. Also, if we add TA's in at this stage, we have to decide in advance how we should allocate them, and make sure that's the best way to do it - Lena
        \item How important is the effort distribution in class for predicting the true grades?
        % Not sure what this means ^ - Lena
        \item How does our method compare with other methods (e.g. taking median, taking average, Piech's method) in terms of error (e.g, mean squared error)
        % keep dataset constant for each comparison, but generate many different datasets
        % how to generate same dataset and test Piech/our method on it? if we test on different datasets then we're not really comparing performance apples-to-apples I think - Lena
        \item How does our method compare with a real TA in terms of error (e.g, mean squared error)
     \end{itemize}
    \item How accurate are the estimated grader performances?
    % What's a good benchmark for estimating grader performances? TODO? Also, median can't estimate grader performances - Lena
    \begin{itemize}
        \item Repeat steps above but this time look at grader performances estimates 
    \end{itemize}
    \item How scalable our method is?
    % Should there be a benchmark for scalability? I think we should test scalability of Piech's method and our method, on real data. IDK about synthetic data - Lena
    % Not sure what the claim here is either, yet
    % Sample claim: memory/time usage does not become exponential with class size, and it's reasonably low (i.e. not days) for an average-sized class? - Lena
    \begin{itemize}
        \item What's the running time of the inference as a function of class size, number of weeks, and grades per submission?
        \item How much memory does it use as a function of class size, number of weeks, and grades per submission?
    \end{itemize}
    
\end{itemize}
 
  \subsection{Real world predictions}
\textbf{Question:} How does our method do on CPSC430 real data in terms of accuracy of estimates?
\begin{itemize}
    \item how did we tune up our hyperparameters (later (or maybe here?) do a sensitivity analysis on these hyperparameters)?
    \item How do we show that we've aggregated grades well?
    \begin{itemize}
        \item hide some observed TA grades and predict them by predicting the true grades; then calculate MSE. (note: we can use new calibrations and TA data and use that information in the paper) % not sure what this means "new calibrations and TA data" - Lena
        \item compare MSE to the median grade or mean or the random walk model vs random walk + censored data vs censored data
        % don't we also want to compare to Piech's method? - Lena
        \item claim that our method is as good as a TA even though a TA would not be great, e.g., calculate TA noise and try to be within a TA noise with inference. 
    \end{itemize}
    \item to show that we've estimated grader performances well
    \begin{itemize}
        \item  use TA spot checked reviews as true labels for effort draws and try to estimate those.
        \item Using Fall18/19 data, run the inference until week $n$ and compare dependability until week $n$ with what the TA said for that particular week's evaluation for a student that is spot checked.
    \end{itemize}
    \item How important is the choice of parameters in estimating true grades and dependabilites? Run sensitivity analysis
    % what is the sensitivity analysis for? what would be a possible claim here? - Lena
\end{itemize}


\subsection{Robustness to misspecification}
\textbf{Question:} Is our model more specified compared to Piech's model?
\begin{itemize}
    \item Step 1:
    \begin{itemize}
        \item Generate data using Piech model
        \item estimate true grades using Piech model and our model
        \item compare estimates
        \item claim that our model either does better or reasonably good on this data
    \end{itemize}
    \item Step 2:
    \begin{itemize}
        \item Generate data using our model
        \item estimate true grades using Piech model and our model
        \item compare estimations
        \item claim that Piech can not aggregate data generated by our model well
    \end{itemize}
\end{itemize}


\subsection{Robustness to student behavior (?)}
% low-effort student behaviour isn't something that a prof using our system can change... unless they use incentives, I guess - Lena

\begin{itemize}
    \item Plot a graph that compares MSE of different models when the number of low effort students decrease.

    \item Potentially a plot that has How many students do the bad behavior vs How much TA is needed
    \begin{itemize}
        \item Argue that if only a few are bad the inference detect this, if a lot of them are doing bad then the spot-checking system would take care of this.
    \end{itemize}

\end{itemize}
\subsection{Evaluate the effect of TAs and calibrations in the system (?)}
This is mostly plausible with synthetic data. 
\begin{itemize}
    \item spot check randomly
    \item spot check based on inference
    % Yeah I feel like maybe TA's should be left out of our experiments until this point... not sure - Lena
\end{itemize}

==> old/inference.tex <==

% no longer closed form updates


\subsection{Technical details of the Bayesian inference method}
\begin{itemize}
    \item Describe the Gibbs sampling algorithm used in running the inference
\end{itemize}
(Refer to the Effort model theory doc.)


==> old/model.tex <==
\gd{Preamble: recap what we're hoping to achieve with this model. It should capture integer-valued grades, low-effort grading behaviour, and grades with multiple components.}
In this section, we define the \emph{binary effort model} (BEM)...

\begin{figure}
    \centering
    \input{figures/model_bem}
    \caption{The BEM graphical model.}
    \label{fig:my_label}
\end{figure}

Following \citet{piech2013tuned}, we suppose that $U$ is a set of assignments and $V$ is a set of graders, consisting of both students and TAs. 
We write $v \to u$ to indicate that an assignment $u \in U$ was graded by a grader $v \in V$.
%The grading rubric consists of $C$ components, each of which can take on values in $\{0, 1,\dots, M\}$.
We consider the following set of latent and observable variables:

% describe variables 
% - true grades
% - reliabilities
% - efforts: clamp to 1 for TAs
% - effort draws
% - observed grades
% - reported grades: round to the nearest reportable value (ex: nearest integer)
\begin{itemize}
    \item \textbf{True grades:} For each assignment $u \in U$ and each rubric component $c \in \{1, \dots, C\}$, there is an underlying \emph{true grade} $s_{u,c} \in \mathbb{R}$.
    % \item \textbf{True grades:} Each assignment $u \in U$ has a vector of true grades $\bm{s}_u \in \mathbb{R}^C$, with separate true grades $\bm{s}_{u,c} \in \mathbb{R}$ for each rubric component $c \in \{1, \dots, C\}$. 
    %is the true grade for rubric component $c$.
    \item \textbf{Grader reliabilities}: Each grader $v \in V$ has a \emph{reliability} $\tau^v \in \mathbb{R}^+$ corresponding to their grading ability, with more reliable students tending to assign grades closer to the true grade. 
    \item \textbf{Grader efforts}: When grader $v$ grades an assignment $u$, they select an \emph{effort} $z_u^v \in \{0, 1\}$.
    If they put in \emph{high effort} ($z_u^v = 1$), they give a grade correlated with the assignment's true grade; if they put in \emph{low effort} ($z_u^v = 0$), they instead ignore the contents of the assignment, giving an uninformative grade (e.g., close to the class average).
    Each grader also has an \emph{effort probability} $e^v \in [0, 1]$, which is the probability that they put in high effort.
    % \item \textbf{Grader efforts}: Each grader $v \in V$ also has an \emph{effort} $e^v \in [0, 1]$, which is the probability that they give an informative grade to an assignment they are grading. 
    % When grading assignment $u$, they select an \emph{effort draw} $z_u^v \in \{0, 1\}$; they give an honest grade if this effort draw is $1$, but choose an uninformed grade independent of the assignment if the effort draw is $0$.
    \item \textbf{Observed grades}: When asked to grade assignment $u$, grader $v$ obtains an \emph{observed grade} $o_{u,c}^v \in \mathbb{R}$ for each rubric component $c \in \{1, \dots, C\}$ of the assignment.
    %, \dots, o_{u,C}^v
    \item \textbf{Reported grades}: Finally, graders use their observed grades to select integer-valued \emph{reported grades} $r_{u,c}^v \in \{0, 1, \dots, M\}$ from the rubric for each component $c \in \{1, \dots, C\}$ of assignment $u$.
\end{itemize}

% TAs and calibrations
We model TAs as graders who have a high (but unknown) reliability. % and always puts in high effort.
We also model calibrations as assignments which were graded by an ``instructor'' grader, who is known to have a very high reliability and always exerts high effort.

% describe BEM model
Specifically, we consider the following generating process:
\begin{alignat*}{2}
    \text{(True grades)}& \quad 
    s_{u,c} &&\sim \mathcal{N}(\mu_s, \tau_s) \\
    \text{(Reliabilities)}& \quad 
    \tau^v &&\sim \GammaDist(\alpha_\tau, \beta_\tau) \\
    \text{(Effort probabilities)}& \quad 
    e^v &&\sim \BetaDist(\alpha_e, \beta_e) \\
    \text{(Efforts)}& \quad
    z_u^v &&\sim \Ber(e^v) \\
    \text{(Observed grades)}& \quad
    o_{u,c}^v &&\sim \begin{cases}
        \mathcal{N}(s_{u,c}, \tau^v), & z_u^v = 1 \\
        \mathcal{N}(\mu_s, \tau_\ell), & z_u^v = 0 \\
    \end{cases} \\
    \text{(Reported grades)}& \quad
    r_{u,c}^v &&=  \begin{cases}
        M, & o_{u,c}^v > M \\
        \round(o_{u,c}^v), & o_u^v \in [0, M] \\
        0 , & o_{u,c}^v < 0 \\
    \end{cases} 
\end{alignat*}


% describe hyperparams
Here, $\mu_s$ and $\tau_s$ are the mean and precision of the true grade prior, $\alpha_\tau$ and $\beta_\tau$ parameterize the grader reliability prior, and $\alpha_e$ and $\beta_e$ parameterize the grader effort probability prior.
The low-effort grading behavior is to choose a grade close to the class average, plus Gaussian noise with precision $\tau_\ell$, and report its rounded value.
\gd{Support this with evidence from class and cite Hartline's scoring rule paper.}

% (figure: graphical model)
\begin{figure}
    \centering
    % \includegraphics{}
    TODO: graphical model?
    \caption{TODO: graphical model caption}
    \label{fig:model}
\end{figure}

% why not model bias?
% why model true grades as reals, not integers?
% What is the "reported grade" layer for? 
\gd{Explain some of our modeling choices here? No bias; real-valued true grades}

% two variants of the model
% - uncensored: treat grades as observed grades (as in Piech and most other work)
% - censored: treat grades as reported grades
Motivated by previous work, we consider one simplification of our model, where we remove reported grades from the model and instead treat the integer-valued reports as real-valued observed grades.
We refer to this variant as the \emph{uncensored BEM}.





% censored PG1
% - also consider similar modification to PG1

% first draft:
%In our model, each assignment $u$ has a \emph{true grade} $s_u \sim N(s_u; \mu_s, \tau_s)$, where $\mu_s$ is the class average and $\tau_s$ is the precision of the grades. Each student $v$ has a \emph{reliability} $\tau^v \sim \text{Gamma}(\tau^v; \alpha_\tau, \beta_\tau)$ and an \emph{effort} $e^v \in [0,1] \sim \text{Beta}(\alpha_e, \beta_e)$. Whenever student $v$ is asked to grade an assignment $u$, they decide an \emph{effort draw} $z_u^v \in \{0,1\} \sim \text{Ber}(e_u^v; e^v)$ . Then, they choose a \emph{reported grade} $r_u^v \sim P(r_u^v; o_u^v, z_u^v)$ based on the following:
%    \begin{itemize}
%        \item If $z_u^v = 1$ (``high effort''), they give $r_u^v = \text{round}(o_u^v)$, where $o_u^v \sim N(o_u^v; s_u, \tau^v)$ is their observed grade when they put in high effort. 
%        \item If $z_u^v = 0$ (``low effort''), they select $r_u^v \sim P_\ell(r_u^v)$ from a predetermined low-effort distribution. 
%    \end{itemize}

%We model TAs as highly reliable students who are always high effort. We also assume that we have set of calibrations for which true grades are known with high accuracy.  We'll also need two more pieces of notation. $I(r_u^v)$ denotes the \emph{interval} of observed grades that would round to the reported grade $r_u^v$. Typically, $I(r_u^v) = [r_u^v - \frac{1}{2}, r_u^v + \frac{1}{2}]$, but it's possible to use different interval sizes. Finally, the random variable $x \sim \text{truncnorm}(\mu, \tau, a, b)$ is drawn from a \emph{truncated normal} distribution with mean $\mu$ and precision $\tau$, subject to the bounds $a \le x \le b$. If $I = [a, b]$, $\text{truncnorm}(\mu, \tau, I)$ is shorthand for $\text{truncnorm}(\mu, \tau, a, b)$ (ie: $N(\mu, \tau)$ truncated to the interval $I$). 


==> old/problem_statement.tex <==
\section{Details of the new grading mechanism}

\subsection{Students' Essay Grade}
\begin{itemize}
    \item After the deadline for submitting student reviews, run Bayesian inference on new and old data points gathered for each student. Use inference output as tentative essay grades.
    \item Once the TA grades are in (either true appeals or spot checks) finalize grades.
    \item Re-calculate them internally only for the sake of calculating more accurate grades for future weeks.
\end{itemize}

\subsection{Students' Weekly Peer Review Grade}
\begin{itemize}
    \item after the deadline for submitting student reviews, run Bayesian inference on new and old data points gathered from each student to calculated tentative effort and reliability estimates.
    \item Calculate the dependability score (this is yet to be defined formally) for each student.
    \item After TA grades are in, re-run inference and finalize dependability of each student for the week that they graded in. 
\end{itemize}

\subsection{Calibrations}
\begin{itemize}
    \item Once a new calibration is submitted:
    \begin{itemize}
        \item think of every other essay grade and dependability as observed except for the student who submitted the calibration
        \item run the inference to re-estimate dependability. 
    \end{itemize}
    \item This is fast because everything else is fixed. The result would mainly affect how student reviews are assigned. 
\end{itemize}


\subsection{Assigning student reviews}
\begin{itemize}
    \item Update beliefs about students' dependability by the essay submission deadline.
    \item Sort them based on that, match students with high dependability with each other.
    \item The exact matching algorithm is flexible. Probably the best way is to put them in a loop and have each student grade the next three students in the loop. 
\end{itemize}
  

\subsection{Assigning TA reviews}
A TA review or spot check consists of 
\begin{itemize}
    \item grading the essay carefully and updating its score.
    \item flagging each review either as high effort or low effort.
\end{itemize}
 The new true grade and information on student effort is then used to update dependability score for each student involved in the essay for that week. 
 
Spot checking budget is divided into three items:
\begin{itemize}
    \item High grades
    \item Random
    \item Submissions that are most likely appealed, e.g., high variance grades
\end{itemize}

\begin{figure*}
    \centering
    \includegraphics{figures/fall19-variance.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure*}

==> outline.tex <==



Solving practical problems with using Bayesian inference in practice. 

discrete grades >> censoring >> maximizing the effect of censoring >> 

study what happens

reported class average

interpret grades

center your thought around the claim and what I can do to support that claim


EC outline (more incentives, less inference)

1 Intro (pitch):
- Main claim is about incentives
    ○ Effort model: inspired by Jason Hartline/Arpita Ghosh
    ○ Interpretability (MIP): a way of understanding the mechanism
    ○ Zombies: gives students a way to influence their rewards in a short time
    ○ TAs: inform spotchecking with confidence intervals (especially on dependability)
    ○ Censored data: helps with incentives of appealing (avoiding appeals to “round up” a grade)

1.1 Related work
- State of the art Bayesian inference models (PG1, Vancouver, GCN)
- Incentive problems in peer grading (from the EC community)
    - put here if talking English is fine
	
2 Bayesian modeling
2.1 Warmup: "standard" PG1 model
2.2 How we adjust it to make BEM
    - Effort
    - Censoring

3 Incentives 
% How the model helps with incentives when using it in a class:
    - Model features
        - Effort
        - Censoring
        - Grading graders
    - Zombies
    - MIP
    - spotchecks/appeals
    
4 Experiments
4.1 Synthetic data
- showing that we actually addressed them
    - true grade accuracy
    - recovering efforts/dependabilities
        - # calibrations/# TA grades, etc
        - Censored data in these too? 
        - (TA spotchecks?)
        - (ways of spotchecking?)
    - MIP doesn't ruin grades
        - Compare grades before and after MIP and show the changes
        - How to tune MIP parameters?
    - Zombies window size
        - show accuracy as a function of window size
    % - (student perceptions? anecdotes from 430?)
    
4.2 Real data
- evidence of the existence of low-effort behavior
    - students with less variance than final grade distribution

- assessing effectiveness of dependability scores
    - low variance graders have low effort, not for Piech [ those same people from above got caught ]
    - high variance graders are caught as unreliable
    - how good are TAs anyway? [Discussion: revisiting clamping efforts to 1?]

- show effectiveness of mixing with uniform?

- experimental setup:
    - where do hyper-parameters come from
    - ...













Introduction:

Peer grading is a wonderful thing
- helps students learn
    - more frequent and faster feedback
    - exposure to work at their own level of competence
    - internalization of the rubric
- helps manage large classes at lower cost

The AI community has recognized the design of peer grading systems as an important problem of interest.

There are two, somewhat interconnected strands of work in the literature:

1. statistical approaches (infer true grade, graders' reliabilities from students' joint reports)

2. peer prediction/mechanism design approaches (particular attention paid to the problem that students don't always have an incentive to report grades honestly; it's less work to do a superficial job grading)

3. of course, there are some lines of work that bring together both elements.

We start from a recent statistical approach and show how it can be advanced both to better model reality and to better reward good behavior and punish bad behavior, thereby bringing in many of the best ideas from the game theoretic literature.

In what follows, we begin by describing a statistical approach to inferring assignment grades and grader reliabilities that roughly follows Piech et al and captures the current state of the art (Section 2). We show how to elaborate this model in three key ways: (1) to perform (better/more reliably?) when grades are discrete instead of continuous; (2) to account for the fact that students may follow low-effort strategies that existing models would otherwise interpret as reliable grading; (3) to allow for the existence of TA graders (who always make an effort) and calibration assignments (whose true grades are already known) to improve the system's estimates of both true grades on student assignments and student reliabilities (Section 3). In Section 4 we explain why this architecture offers good incentives, particularly when combined with an appeal mechanism and TA spot checking. In Section 5 we present experimental data that shows the quantitative performance of our system. .....

---
Section 2: Existing state of the art

Piech model (whatever version of it we actually use).

Explained via a graphical picture.

How does inference work.

Maybe: some problems with it. Or, maybe give these in Sec 3 also
- rounded grades can show high agreement -> high reliabilities

---

Section 3: Methods

3.1 Censoring
  - model
  - inference
  - describe the inference problem this solves 

3.2 Low effort
  - model
  - uncensored inference
  - censored inference

3.3 TAs and calibrations

---

Section 4: Incentives

4.0 Do we want to talk about zumbies and MIP stuff here?

4.1 Grading graders

The core of an incentive scheme is to explicitly give students a grade for grading. How do we do this. Confidence interval; prior. Show that this score goes up with reliable grading, and also that students can improve their grade by doing more calibration.

4.2 Appeals

If someone gives another student a low grade, they will be reported. 

4.3 Spot checking

If someone gives another student a high grade, they might not be reported. Spot check these more. Also spot check other problematic cases; explain our various logic. Describe how TAs grade effort, but not reliability.

4.4 The problem of reporting the mean

Jason Hartline: students look pretty reliable when they report the mean.

Our solution: explicitly model this possibility, prior prefers it to effortful grading

Under our grading scheme described above, and with the mechanism where TAs observe effort (partly based on signals that live outside the model like the text of a review) this attack is no longer effective.

Arpita-style argument that no other attack is easy to carry out/focal?

----

Section 5: Synthetic data

    - scaling studies
        - how many samples does it take? How do you determine?
        - how is runtime as a function of class parameters? ("can I use this in my class?")

    - recovering inference parameters (as a function of class parameters)
        - what influences our ability to recover true grades?
            - scaling grades per assignment: BEM surpasses TA with 4 assignments; other methods need 6
            - TA grades: need ~1/3 of the class to be graded by TAs to match BEM's improvement
        - ...our ability to recover reliabilities/efforts?
            - scaling grades per student: more data per student helps censored BEM recover efforts
            - TA grades: adding a few TA grades helps recover reliabilities (makes sense they need to grade effort outside of the model)
            - calibrations: grading a few calibrations also helps with reliabilities and efforts

    - robustness to misspecification
        - wrong hyper-parameters (which ones matter?)
            - class average: getting low-effort distribution wrong makes a big impact on effort estimates
            - class grade variance: big impact on true grade estimates (why?); too small is bad for reliability estimates
            - reliability prior: extreme values ruin reliability and effort estimates, but generous range of good priors
            - effort prior: only affects effort estimates in uncensored BEM
            - low effort precision (needs correct range): too uniform makes everything worse; too concentrated makes uncensored BEM worse
        - wrong generating process (data from PG1)
            - over range of TA grades: (un)censored BEM recovers true grades and reliabilities as well as PG1
            - (grades per assignment: still running)
            - (stretch goal: how can it do this?)
        - how much of a difference does the censored model make? (stretch goal: okay to describe conceptually in section 3)
            - one lucky grade difference

----

Section 6: Real data

    - evidence of the existence of low-effort behavior
        - students with less variance than final grade distribution
    
    - show effectiveness of mixing with uniform?

    - experimental setup:
        - where do hyper-parameters come from
        - ...
 
    - assessing effectiveness of dependability scores
        - low variance graders have low effort, not for Piech [ those same people from above got caught ]
        - high variance graders are caught as unreliable
        - how good are TAs anyway? [Discussion: revisiting clamping efforts to 1?]

        
    
    






==> related_work.tex <==
%Our methods draw from two lines of work in the peer grading literature: graphical models of peer grading, and the existence of strategic behavior in peer prediction systems.



%\paragraph{Alternative grade aggregation methods.}


%Notably, 
%\citet{fang2017rankwithta} propose an iterative method to estimate true grades, weighting an assignment's peer grade by the grading accuracy of each grader calcualted from the previous iteration. 
 %This work is similar to ours in that it uses input from TAs and instructors as a signal about students' performance. 

%Two recent closely related papers estimate grader biases and reliabilities an a way that seeks to strengthen the incentives offered to students~\citep{prajapati2020swagrader, chakraborty2018incentivizing}. The key idea is a ``social welfare score'' that measures the (beneficial or harmful) influence of a particular grader on the class. This work is similar to ours in the sense that it is based \cite{piech2013tuned} and is concerned with incentives, but we take a different approach to avoid low effort behavior in our system. 

% Main related work categories:


% \subsection{Probabilistic Modeling}
% The closest line of work to ours focuses on using probabilistic modeling, Bayesian inference, and machine learning to improve grading accuracy in peer grading systems. %~\cite{piech2013tuned,raman2014methods, shah2014some, labutov2017jag, sajjadi2016peer, kulkarni2014scaling, wang2019sspa, yuan2020practical, walsh2014peerrank,mi2015probabilistic, fang2017rankwithta, wang2019improving, namanloo2021improving}.
% The most influential work in this area is that of \citet{piech2013tuned}, which proposes three closely related graphical models for peer grading, termed PG1, PG2, and PG3. PG1 attributes a latent bias and reliability parameter to each student and a latent true grade to each assignment and estimates these parameters through Bayesian inference. The bias parameters specify the tendencies of individual students to be easy or hard graders; the reliability parameters model the inherent noise arising from each student's grading ability.  PG2 extends PG1 by assuming that the biases of students take a random walk as students do more grading. PG3 assumes that the reliabilities of students are correlated with their true grades. %\klb{move this}In our experiments with PG1 on our real class data, we observed it inferred very small bias terms overall. We think that this because early in the course, we ask students to grade a set of carefully graded calibration assignment, which would reduce any biases that they have. However, we have also observed that only modeling reliabilities does not explain some of the behaviors that we see in class. 

% % We use PG1 without biases as the base on our work because (1) we think that after students are calibrated in the system, the effect of biases (and their random walk) would be negligible and (2) we want the incentives for grading to be independent of assignment grades. %\hz{discuss bias here}%Overall, our model differs from PG1 in the following ways: (1) we take incentives or effort into account; (2) we do not include student biases in our model since we think that after students have gone through calibration mechanism, their biases would be significantly reduced; (3) our model handles the fact that students can only report inter-valued grades to the model. 
 
%  Inspired by~\citet{piech2013tuned}, various follow-up work focused on designing modified models to improve predictive accuracy. Notably, PG4 and PG5 extend PG3 by assuming that there is a probabilistic
% relation between graders reliabilities and their true grades, i.e., they assume that students with higher grades are better graders. PG6 and 7 extend PG4 and 5 by feeding the difference between grades into the their Bayesian network as well. 
 
%  %\citep{sajjadi2016peer,yuan2020practical,mi2015probabilistic,wang2019improving}. 

 
%  %. Their approach is similar to our work in the sense that it gives less weight to unreliable grading behavior. But, , 
 

% \subsection{Iterative approaches}

% There is a line of work in the literature that focuses on aggregating grades and incentiving high quality grading as point estimates using iterative approaches~cite(walsh and Vanvouver). In these approaches, the final grade of each assignment is set to be the weighted average of its reported grades, where the weight of each reported grades reflects the accuracy of the grader who submitted the grade. The grading accuracy for each grades reflect at each step reflects how far reported grades are from what the algorithms thinks about the true grade at each step. If TA grades are available these grades are always used at final true grades.  A nice property of such approaches is that they produce interpretable grades. However, they produce point estimates which does give much information about how confident the method is about each grades. They also do not handle discrete grades properly. 

% These approaches also suggest to use the estimates for grading accuracy as part of each students final grades so that students are encourage to put in the effort for grading better.

%  %For example, \citet{fang2017rankwithta} propose an iterative method to estimate true grades, weighting an assignment's peer grade by the grading accuracy of each grader calcualted from the previous iteration. 
%  %This work is similar to ours in that it uses input from TAs and instructors as a signal about students' performance. 
 
 
% % They explore two approaches regarding TAs: (1) where a TA is treated as a skillful student, and (2) where TA grades are used to estimate student biases before aggregation. Similarly, we model TAs as high reliability graders who always make an effort, leveraging this signal to obtain better estimates of the model's remaining parameters.
 
 
%  %\citet{raman2014methods} explores several probabilistic rank aggregation models and shows the efficacy of this type of grade aggregation compared to cardinal peer grading and traditional evaluation techniques. The main way in which their work differs from ours is that it uses peer grades in an ordinal, rather than cardinal, form. However, the overall objective of accurate peer grade aggregation aligns with our own.

% % Peer prediction approaches

% % 




% % There are two interconnected strands of work in the literature that closely relate to our work: mechanism design approaches, which focus on the problem that students do not always have the incentive to put in high effort to grade their peers accurately; and statistical approaches, which focus on inferring true grades and graders' reliabilities based on students' grading behavior.

% \subsection{Incentives and modeling student effort}

% There is a prominent line of work in the mechanism design literature focusing on incentivizing high quality grading in environments such as peer grading and reviewing~\citep{liu2018surrogate,goel2019deep, faltings2012eliciting,prelec2004bayesian,radanovic2014incentives,riley2014minimum,witkowski2012robust,witkowski2013dwelling,jurca2009mechanisms,kong2016putting,jurca2005enforcing,kamble2015truth,radanovic2013robust,shnayder2016informed, gao2019incentivizing,zarkoob2020report}.
% Work in this area is mostly centered around the idea of peer prediction.
% In such mechanisms, students (agents) are incentivized to behave honestly based on how their behavior compares to their classmates. 
% A common issue associated with most peer prediction mechanisms is that they rise to uninformative equilibria in which students would prefer to game the system by reporting uninformative grades~\citep{jurca2009mechanisms,witkowski2013dwelling,kong2016putting,shnayder2016informed,dasgupta2013crowdsourced,gao2019incentivizing,zarkoob2020report}. 
% Much of the work in the peer prediction literature focuses on using mechanism design and statistical methods to obtain incentive mechanisms that do not suffer from uninformative equilibria~\citep{liu2018surrogate,goel2019deep}. 
% While such attempts are mostly orthogonal to this work, modeling low-effort behavior in our models is partly motivated by the existence of uninformative behavior by students in a peer grading environment.

% %\gd{Too much detail?}

% \subsection{Other closely related work}

% Recent work by \citet{burrell2021measurement} discusses the importance of measuring effort in peer grading settings and focuses on the question of how to grade the graders. In their model of peer grading, grades are discrete and effort is defined as the number of draws that each grader obtains from a latent binomial distribution that is specified by the grader bias and the true grade distribution. %They also look into PG1~\gd{We haven't said what this is yet.} as the continues version of their model and consider reliability as the equivalent to their effort level. 
% They experiment with using a variety of out-of-the-box peer prediction mechanisms to reward graders, finding that these peer prediction reward functions do not accurately reflect grader effort levels. 
% %(or reliability in the case of PG1) used to generate the data. 
% In contrast, we use a simpler model of grader effort in which graders make binary effort decisions.
% We treat discrete-valued grades as censored data, allowing us to perform inference on them, and focus on our models' abilities to correctly aggregate true grades. 
% % Our work uses a similar model of grader effort, 
% % Their model of effort is different from ours and is not applicable to our setting. Also, they are not at all concerned with aggregating reported grades to estimate true grades. %In contrast, we start from PG1 and explicitly integrate efforts into it. This helps us to estimate true grades better in the presence of such low effort behavior and also gives us a reliable way to grade the graders.
% % Also, we handle discrete grades by thinking about reported grades as censored data. 
 

 
% Finally, two recent papers extend \citet{piech2013tuned}'s PG1 model to estimate grader biases and reliabilities an a way that seeks to strengthen the incentives offered to students~\citep{prajapati2020swagrader, chakraborty2018incentivizing}. The key idea is a ``social welfare score'' that measures the (beneficial or harmful) influence of a particular grader on the class. This work is similar to ours in the sense that it extends \cite{piech2013tuned} and is concerned with incentives, but we take a different approach to avoid low effort behavior in our system. We do not see how its incentive properties could be tested without deploying it in practice, which we did not do, and so we do not evaluate it in this paper.


% \subsection{Ordinal approaches}

% There is a line of work that does peer grading in a world where graders are asked to compare the submissions that they are assigned to grade and give an ordering over them~\cite{shah2013case,mi2015probabilistic,raman2014methods}. These partial orderings are then merged to obtain a total ordering over all the submissions and is used to assign final grades to students' submissions. The work in this area argues that ordinal approaches work better in practice because it is easier for students to compare submissions and say which ones better that the other rather than assigning a raw numerical value to their quality. However, \cite{de2014crowdgrader} mentions that students reported uneasiness to rate their peers. Furthermore, we believe that the presence of calibration assignments should make easy the concerns over having students assigning numerical grades to their peers. 


%~\citet{lu2015grading} studies look into whether the following factors incentivize students to make an effort during peer grading: (1) knowledge that you are being graded, and/or (2) the opportunity to evaluate other students' peer grading. The position was taken that it seemed counterproductive to reward or punish good grading since students are simply there to learn the material, not to learn to grade. It was found that when students were shown evidence that their peers are producing high-quality grading, then this motivates them to do the same. This paper, by comparison to our work, examines incentives rather than peer grade aggregation and presents a novel view of them.


 
% - Papers that implement various peer grading systems
 
% \textit{ComPAIR: A New Online Tool Using Adaptive
% Comparative Judgement to Support Learning with Peer
% Feedback} ~\cite{potter2017compair} -- In this paper's experiment, students are shown increasingly similar assignments from their peers and asked to rank them along several dimensions. Results show perceived learning benefits of the system. No focus is given to crowdsourcing, grade aggregation, or training students to grade better. The clearest difference between this study and our work is the paper's focus on student experience rather than peer grade aggregation.
 
 
 
 
 
 
 %This procedure is compared to PeerRank ~\cite{walsh2014peerrank} using tests on synthetic data, and while both methods perform far better than aggregation using the average, RankwithTA outperforms PeerRank slightly.


% In~\citep{wang2019sspa} grade aggregation of peer grades is done using similarity measures of peers to each other, and to the instructor. This work is similar to our work in that it assigns to each assignment a weighted average of the graders' reports. However, the weight for each grader is computed to be a similarity measure (between 0 and 1) between this grader and a TA or instructor. This paper shows on Sajjadi's dataset ~\cite{sajjadi2016peer} an improvement to using the average for grade aggregation.
 
%  \begin{itemize}
%  \item \textit{Tuned Models of Peer Assessment in MOOCs} ~\cite{piech2013tuned} -- Piech
 
%   \item \textit{Methods for Ordinal Peer Grading} ~\cite{raman2014methods} -- This paper gets students in MOOCs to perform comparisons (ordinal peer grading) as opposed to absolute rankings of assignments, since it is shown to be easier to do. They also explore several probabilistic rank aggregation models, and show the efficacy of this type of grade aggregation compared to cardinal peer grading and traditional evaluation techniques. The main way in which this work differs from ours is that it uses peer grades in an ordinal, rather than cardinal, form. The overall objective of accurate peer grade aggregation aligns with our own.
 
 
%  \item \textit{Some Scaling Laws for MOOC Assessments} ~\cite{shah2014some} -- As class size increases, a theorem is posited that fixed proportion of students will make grading errors. This paper uses dimensionality reduction and clustering to allow the fraction of errors to go to zero as the class size grows. In effect, a grade aggregation technique via clustering can be used to prevent assignments from being given final grades that are incorrect. This technique is introduced theoretically, but not tested empirically, but both this work and ours is focused on improving the accuracy of peer grade aggregation methods.

% \item \textit{JAG: A Crowdsourcing Framework
% for Joint Assessment and Peer Grading} ~\cite{labutov2017jag} -- this paper frames peer grading as the answering of multiple-choice questions (MCQs) for which the answer key is not known, with two possible answers for each question. They construct a probabilistic model with student ability and question difficulty, which is then fit using EM. This model does not take into account incentives or effort, since they assume that a (relatively) low-ability student will simply guess an answer to each MCQ. This model is not suitable for our use, since assignment grades that are real values may admit grading strategies that would not make sense for a multiple choice test. Furthermore, this model differs from ours in that it only admits two possible answers for each MCQ.

% \item \textit{Peer Grading in a Course on Algorithms and Data Structures:Machine Learning Algorithms do not Improve over Simple Baselines} ~\cite{sajjadi2016peer} -- in a computer science class, a probabilistic model based on~\cite{piech2013tuned} was used to predict the true grades of assignments, and compared to several other aggregation methods. TA's were taken as ground truth, and it was found that taking the mean did not improve over using~\cite{piech2013tuned}'s probabilistic model. This paper's did not propose or test an effort-based model. In comparing ordinal ranking algorithms and the bias-reliability model, it was found that in almost all cases, both algorithms performed worse than simply taking the mean. One of the likely reasons for this is the nature of grading error -- it was very easy for students to miss a single error in a question while marking, and give a substantially higher mark than deserved. As we are testing on essays, it is possible that grading error will be more adherent to model assumptions in our case.

% \item \textit{Scaling Short-answer Grading by Combining Peer
% Assessment with Algorithmic Scoring} ~\cite{kulkarni2014scaling} -- instead of aggregating peer grades, an algorithm first determines how many peer graders to assign to an assignment. Then, based on how much  agreement there is between these peers, the mechanism may add more peers to grade the assignment. This method was shown to perform better than using the median for grade aggregation. This method is quite different from ours in that it uses NLP to direct the amount of peer assessments an assignment gets. It assumes simple answers to the assignments, either binary answers or enumerative short answers. Its method of aggregation is based on several peers independently reaching the same consensus in their marking.

% \item \textit{Practical Methods for Semi-automated Peer Grading
% in a Classroom Setting} ~\cite{yuan2020practical} -- This paper builds upon Piech and other peer grade aggregation mechanisms by using the idea of bias. However, instead of estimating it using Gibbs sampling from a probabilistic model, bias is estimated only from calibrations. Finally, the quality of reviews is estimated from the content of the review itself; this review quality is then used to give some reviews more or less influence on the final grade. Several methods are used to estimate the quality of reviews: review length as well as language models. This work is very similar to ours, but neglects to take into account the possibility of low-effort behaviour in students, whether through an explicit model, or through incentives.

% \item \textit{The PeerRank Method for Peer Assessment} ~\cite{walsh2014peerrank} -- This method uses an iterative procedure similar to PageRank to estimate grader reliability. It is very similar to the PG3 model that Piech describes in their paper. This approach ties the grade that a paper gets to the ability of the grader, which creates an incentive for each grader to grade as accurately as possible. The PeerRank method outperforms the average in experiments on synthetic data. We do not believe that both the grade a student obtains and this student's grading ability should be represented by one value, so we do not take the approach investigated by this paper.

% \item \textit{Human-machine hybrid peer grading in
% SPOCs} ~\cite{han2020human} -- This paper argues that Bayesian models such as those developed by Piech perform worse on small classes (SPOCs) than on MOOCs. For smaller classes, random or unreliable grading behaviour is more of a problem during grade aggregation. Methods are proposed in order to filter the peer grades before applying grade aggregation frameworks to them. These methods range from naive Bayes to CNN's, and use the text itself to assign a score to the assignment. The system then discards any peer grade that is further from this score than a predefined threshold. When tested on a real class and compared with other probabilistic models, this paper's method acheives a much lower RMSE. This work is different from ours in that it integrates automated grading into the system, and does not innovate on the probabilistic model, but our idea of identifying low-effort students and letting them have less influence on the final grade is similarly motivated.

% \item \textit{Probabilistic Graphical Models for Boosting
% Cardinal and Ordinal Peer Grading in MOOCs} ~\cite{mi2015probabilistic} -- This work extends Piech's work via new, related models called PG4 and PG5. They expand on Piech's PG3 model, where a student's reliability is a deterministic linear function of the true grade a student got. However, they do not believe that this function is truly linear, or that it is deterministic. This work reintroduces reliability as a random variable, but explores variations on the distribution it comes from. PG4 sets the reliability as being sampled from the Gamma distribution, with shape determined by the true grade. PG5 sets the reliability to be sampled from a normal centered at the true grade. PG4 and PG5 perform better than the original PG1-3 on a dataset with approximately 7 thousand peer grades. This paper also compares the aggregation of cardinal and ordinal peer grades. The approach taken in this work is very similar to ours, but we do not believe that linking peer grading ability and score on an assignment would accurately reflect the score the assignment should obtain. Moreover, the problem of explicitly capturing effort (or incentivizing it) is not within the scope of the paper.

% \item \textit{Improving Peer Assessment Accuracy by Incorporating
% Relative Peer Grades} ~\cite{wang2019improving} -- This work is motivated by the observation that relative peer grades (the difference in peer grades given by one student to two different assignments) are robust to that student's bias. The authors extended PG1-3 of Piech's work to account for relative peer grades in three more probabilistic models. It was found that by RMSE measures, these new models outperformed Piech's three models. This work is similar to our work in its approach, but there is still the question of why relative peer grades are not already   implicitly accounted for in Piech's models. Also, this work does not concern itself with effort models or incentives.


%  \end{itemize}
 



